Efficient Temporal Pattern Mining in Big Time Series Using Mutual Information -- Full Version

Very large time series are increasingly available from an ever wider range of IoT-enabled sensors deployed in different environments. Significant insights can be gained by mining temporal patterns from these time series. Unlike traditional pattern mining, temporal pattern mining (TPM) adds event time intervals into extracted patterns, making them more expressive at the expense of increased mining time complexity. Existing TPM methods either cannot scale to large datasets, or work only on pre-processed temporal events rather than on time series. This paper presents our Frequent Temporal Pattern Mining from Time Series (FTPMf TS) approach which provides: (1) The end-to-end FTPMf TS process taking time series as input and producing frequent temporal patterns as output. (2) The efficient Hierarchical Temporal Pattern Graph Mining (HTPGM) algorithm that uses efficient data structures for fast support and confidence computation, and employs effective pruning techniques for significantly faster mining. (3) An approximate version of HTPGM that uses mutual information, a measure of data correlation known from information theory, to prune unpromising time series from the search space. (4) An extensive experimental evaluation showing that HTPGM outperforms the baselines in runtime and memory consumption, and can scale to big datasets. The approximate HTPGM is up to two orders of magnitude faster and less memory consuming than the baselines, while retaining high accuracy.

==> Introduction-20210913.tex <==
\vspace{-0.05in}
\section{Introduction}
Rapid advancements in IoT technology have enabled the collection of enormous amounts of time series at unprecedented scale and speed. For example, modern residential households are now equipped with smart meters and smart plugs to enable fine-grained monitoring on the energy usage of the electrical appliances, weather stations have thousands of sensors to monitor hundreds of different weather-related variables, and mobile devices carry various sensors to track user behaviors and locations. These IoT-based systems are generating terabytes of data daily that contain rich information and once unlocked, can offer new insights into the application domains to support evidence-based decision making and optimization. %Analyzing these massive, heterogeneous and rich time series can uncover hidden patterns and extract new insights to support evidence-based decision making and optimization. 
%These massive and heterogeneous time series contain rich information that once unlocked can offer invaluable insights into the application domains to support evidence-based decision making and optimization.

One of the first steps to uncover hidden patterns and extract new insights from time series data is to analyze patterns from them. Consider for example the time series in Fig. \ref{fig:TimeSeries} that shows the energy usage of electrical appliances in a residential household. %Such time series can be analyzed to identify how residents are interacting with electrical appliances to understand their living habits. 
From Fig. \ref{fig:TimeSeries}, a pattern of activations between Clothes Washer, Dryer and Iron can be identified, showing that these appliances are often used together, usually on Wednesday and Saturday evening. 
%From Fig. \ref{fig:TimeSeries}, a pattern of activations between Kitchen, Toaster and Microwave can be identified, which shows that these appliances are often used together, usually in the early morning and evening. 
%showing that these devices are often used together, usually in the early morning and evening. Such insights are important, as they can be used to enable the building of smart houses, and/or optimize residential energy usage. \textcolor{red}{\bf Fixed for R1.} \textcolor{red}{For instance, knowing that a resident always showers at 6:00 would enable pre-heating of hot water, e.g., when surplus wind energy is available, or identifying that a resident has a daily return at 16:00 from work (based on the activation of lights in the hall entry) would enable the creation of inference rule of when to pre-activate the heater.} 
%While time series analysis has been studied extensively in the past, its importance and value only continue to grow. One of the first steps to harness the enormous potential from modern big time series is to discover correlations among heterogeneous and cross-domain datasets. Consider for example the NYC Open Data \cite{nycopen} with more than 1,500 published datasets containing quantitative data from different domains, including weather and transportation, energy and environment etc. Cross-domain analysis among these datasets can reveal new insights about the city and its citizens, and thus aid policy makers in decision making. 
Extracting such patterns is the task of pattern mining. However, traditional pattern mining methods do not fully capture the temporal dimension of the data. For example, sequential pattern would express the relation between appliances in Fig. \ref{fig:TimeSeries} as \{\textit{Washer On}\} $\Rightarrow$ \{\textit{Dryer On, Iron On}\}, %indicating that the occurrence of \{\textit{Dryer On, Iron On}\} is associated with the occurrence of \{\textit{Washer On}\}. 
indicating only the sequential occurrences of the events. 
Such patterns omit the pattern \textit{occurrence times} which contain important information. 
To overcome this limitation, %a recent trend in pattern mining tries to add temporal aspect into extracted patterns, forming a group of methods called \textit{temporal pattern mining}
\textit{temporal pattern mining} (TPM) adds the temporal information into the patterns, and thus, provides further details on when the relations between events happen, and for how long. %In TPM, event occurrences are associated with time intervals, and thus, their relations are enriched with temporal information. 
%Using TPM, the previous pattern can be expressed as: [06:00,07:00] \textit{Kitchen On} $\Rightarrow$ [06:01,06:45] \textit{Toaster On} $\Rightarrow$ [07:00,07:10] \textit{Microwave On}, or [1 hour] \textit{Kitchen On} $\Rightarrow_{\text{after 1 min}}$ [44 minutes] \textit{Toaster On} $\Rightarrow_{\text{after 15 min}}$ [10 minutes] \textit{Microwave On}. This type of patterns provides further details on when the relations between events happen, and for how long, making temporal patterns more informative and expressive. 
For example, TPM can express the previous pattern more informatively as: 
[16:00, 17:30]\textit{Washer On} $\Rightarrow$ [17:35, 19:35]\textit{Dryer On} $\Rightarrow$ [20:30, 21:00]\textit{Iron On}. %or [1.30 hours]\textit{Washer On} $\Rightarrow_{\text{after 5 mins}}$ [2 hours]\textit{Dryer On} $\Rightarrow_{\text{after 55 mins}}$ [30 mins]\textit{Iron On}. 
%This type of patterns provides further details on when the relations between events happen, and for how long, making temporal patterns more informative. 
\begin{figure}[!t]
	\vspace{-0.05in}
	\resizebox{0.85\columnwidth}{!}{\input{data/tikz/timeSeries_Using}}
	\vspace{-0.2in}
	\caption{Energy usage time series of electrical devices}
	\label{fig:TimeSeries}
	\vspace{-0.2in}
\end{figure}

Temporal patterns can be found in most time series data from single or cross-domains. We demonstrate their usefulness below. % of temporal patterns using two examples below. %Analyzing such patterns can enable actionable intelligence which we demonstrate with $2$ examples below.} 

{\color{red} \textbf{Need to be changed.}} {\color{blue} Example 1. In the energy domain, analyzing temporal patterns from residential energy usage time series can reveal how residents interact with electrical devices, and from that, understand their living habits. This allows to optimize the energy consumption. For example, knowing that the group of appliances \{Clothes Washer, Dryer, Iron\} are often used together at [16:00-21:00] every Wed and Sat would allow to automatically shift the operations of the Clothes Washer and Dryer to a time when the CO2 intensity of the electricity is low, e.g., due to large available amounts of solar or wind power, and do the ironing afterwards. This will (typically) reduce both electrical cost and CO2 emissions.}  
	
{\color{red} \textbf{Need to be changed.}} {\color{blue} Example 2. In the smart city domain, temporal patterns extracted from joined weather and traffic time series can reveal the connection between weather conditions and collision severities. For instance, if a pattern: \textit{[15:00, 17:00] Heavy Rain} $\Rightarrow$ \textit{[16:30, 19:00] High Motorist Injury} is found with high confidence, then there is an increased risk of accidents after a heavy rain. Such patterns can assist to warn the drivers and thus reduce accidents.} 

%Temporal patterns mining (TPM) is one of the significant branches in time series analysis. The traditional data mining methods usually ignore temporal dimension, TPM on time series explores relations among events in which temporal dimension is treated explicitly. Fig. \ref{fig:TimeSeries} is an example of time series data of three appliances in energy consumption. The appliances are turned on and off at various time intervals. Mining temporal patterns on this data can discover the interesting temporal patterns. For instance, Toaster and Microwave are turned on while Kitchen is activating. From the discovered patterns, we can predict when to turn on or off certain appliances to save power when not used. This paper concerns efficient temporal patterns mining from big time series, which contributes optimization algorithms of temporal patterns mining, proves the theory of the proposed algorithm, and is applied in many smart applications.  

%Mining temporal patterns from time series can offer valuable knowledge into their domains. For instance, temporal patterns can reveal the connection between weather conditions and collision severities. If a pattern \{[2 hours] Heavy Rain $\Rightarrow$ High Motorist Injury\} can be found with high confidence, we can conclude that there is an increasing risk of accidents after a heavy rain. %Or, the pattern \{[6 hours] Heavy Snow $\Rightarrow $ High Collision\} can suggest authorities to send a warning to drivers after a heavy snowfall. 
%Such patterns can help identify the causes of accidents, and in turn, to warn the citizens. 
%In the energy domain, temporal patterns extracted from energy consumption of electrical appliances can provide insights into the living habits of residents, and the way electrical appliances are being used in residential households. Such insights are important, as they can be used to enable the building of smart houses, or optimize residential energy usage. For example, knowing that a resident always showers at 6:00 would enable pre-heating of hot water, e.g., when surplus wind energy is available. 

%\textit{To remove this paragraph if space cannot be saved elsewhere.} In TPM, event occurrences are associated with time intervals. This temporal information enables forming complex relations between events. Based on event time intervals, it is possible to identify whether an event occurs following another event, or if their occurrences overlap or contain each other. Such information can be used to form a chain of event occurrences, which is very useful, for instance, in the medical domain to distinguish one disease from another. As an example, knowing that %a patient has a fever occurring first, then overlapped by a dry cough would suggest he/she is more likely to have COVID-19 than normal flu. Or, if there is a decrease of platelet counts on the third day after the onset of a fever would suggest dengue fever is more likely. TPM is also more effective than sequential pattern mining in identifying seasonal patterns. For example, item sales only during Christmas will not be frequent if considering sales data for the entire year, and are thus omitted by sequential mining. Using TPM, these patterns can be extracted by identifying the time of sale events, and then considering their frequency only during the sale seasons. 

Although temporal patterns are useful, mining them is much more expensive than sequential patterns. Not only does the temporal information adds extra computation to the mining process, the complex relations between events also add an additional exponential factor O($3^{h^2}$) to the complexity O($m^h$) of the search space ($m$ is the number of events and $h$ is the length of temporal patterns), yielding an overall complexity of O($m^h3^{h^2}$) {\color{blue}(see Lemma \ref{lem1} in Section \ref{sec:2freq} and the proof in \cite{ho2020efficient})}. %The two main factors that drive the TPM complexity are the number of events which can be converted into the number of data attributes, and the number of temporal sequences (details discussed in Section \ref{sec:FTPMfTSMining}). %thus significantly increasing the mining complexity. 
Existing work such as \cite{tpminer,ieminer,hdfs}, has tried to either use different representations to reduce the relation complexity, e.g., augmented representation, or propose different optimizations to improve TPM performance. However, these methods do not scale on big datasets, i.e., many time series and many sequences, %as the challenge of the exponential search space still exists, 
and/or do not work directly on time series but rather on pre-processed temporal events. %Often, they assume that databases of temporal events are already available, and temporal patterns will be extracted directly from there. To the best of our knowledge, there is no existing work that offers a complete solution to extract temporal patterns from raw time series, as given in Fig. \ref{fig:TimeSeries}.

\textit{Contributions.} In this paper, we present our comprehensive Frequent Temporal Pattern Mining from Time Series (FTPMfTS) approach which overcomes the above limitations. %We provide the following key contributions. 
Our key contributions are:
(1) We present the first end-to-end FTPMfTS process that receives a set of time series as input, and produces frequent temporal patterns as output. Within this process, a splitting strategy is proposed to convert time series into event sequences while ensuring the preservation of temporal patterns.
%(2) \textbf{We should discuss whether this is a key contribution or not.} We provide a formal definition of temporal patterns through event instances, thus provide a more precise representation of the relations between events. %Moreover, we simplify Allen's relation model for better usefulness and extend it with a buffer-based solution to solve the exact time mapping problem, while ensuring that temporal relations are mutually exclusive. 
(2) We propose an efficient Hierarchical Temporal Pattern Graph Mining (HTPGM) algorithm to mine frequent temporal patterns which has several important novelties. First, HTPGM employs efficient data structures, Hierarchical Pattern Graph and \textit{bitmap}, to enable fast computations of support and confidence. Second, two groups of pruning techniques based on the Apriori principle and the transitivity property of temporal relations are proposed to enable faster mining. 
(3) Based on {\color{blue} the concept of mutual information which measures the correlation among time series}, we propose a novel approximation version of HTPGM that prunes unpromising time series to significantly reduce the search space. The approximate HTPGM can scale on big datasets, i.e., many time series and many sequences. 
(4) We perform extensive experiments on synthetic and real-world datasets from various domains which show that HTPGM outperforms the baselines in both runtime and memory usage. The approximate HTPGM achieves up to $2$ orders of magnitude speedup w.r.t. the baselines, while obtaining high accuracy compared to the exact HTPGM.

\textit{Paper outline.} Section \ref{sec:relatedwork} covers related work. Section \ref{sec:preliminary} defines the problem. Sections \ref{sec:FTPMfTSMining} and \ref{sec:MI} present the exact and the approximate HTPGM. Section \ref{sec:experiment} shows the experimental evaluation and Section \ref{sec:conclusion} concludes the paper and points to future work.

%(1) We present the first end-to-end FTPMfTS process that receives a set of time series as input, and produces frequent temporal patterns as output. Within this process, we provide a formal definition of temporal patterns that is defined through event instances, and thus, providing a more precise representation of the relations between events. Moreover, while adopting Allen relation model to represent relations between temporal events, we simplify them, and propose the use of a buffer $\epsilon$ to solve the exact time mapping problem while ensuring the mutually exclusive property of temporal relations. (2) We propose an efficient Hierarchical Temporal Pattern Graph Mining (HTPGM) method to efficiently mine frequent temporal patterns. HTPGM has several important novelties. First, HTPGM employs efficient data structures, Hierarchical Pattern Graph and \textit{bitmap}, to enable fast computations for support and confidence of temporal patterns. Second, two groups of pruning techniques based on the Apriori principle and the transitivity property of temporal relations are introduced in HTPGM to achieve faster mining. (3) Finally, Based on mutual information, we derive the lower bound of confidence of temporal events, and based on that, to approximate HTPGM. This approximation can prune unpromising time series, and thus, significantly reduces the input size, allowing HTPGM scale on big datasets. the most novel contribution of HTPGM comes from an approximation based on mutual information (MI). Particularly, we derive a theoretical connection between MI and the confidence of temporal events, from which an approximation of HTPGM is proposed to prune unpromising time series, and thus, significantly reduces the size of inputs. This approximation helps HTPGM scale on big datasets. We perform extensive experiments on real-world datasets to show that HTPGM outperforms the baselines, with the approximate solution can achieve up to $3$ orders of magnitude speedup, consume less memory, and obtain high accuracy compared to the exact solution.

%To the best of our knowledge, our solution is the first that works directly on time series.  

%We propose a novel approach using mutual information to mine temporal patterns efficiently in time series. We present an algorithm OpTPM that applies three optimization techniques composing the transitive property of relations among events, the Apriori principle, and all-confidence properties. This proposal reduces the complex relations generation and assists in accelerating TPM process. Then, based on OpTPM, we propose a novel algorithm NMICTP using normalize mutual information to eliminate time series which do not satisfy a predefined information threshold. NMICTP prunes many uncorrelated temporal patterns and improves the performance of TMP.

%\textit{Contributions.} Our key contributions are follows.
%\begin{itemize}
%	\item We propose the first solution, FTPMfTS, to mine temporal patterns directly from time series.
%	\item We provide a formal definition of temporal patterns defined through event instances, and thus, providing a more precise representation of the relations between events. 
%	\item We simplify Allen relations, and use a buffer $\epsilon$ to solve the exact time mapping problem, while ensuring the mutually exclusive property of temporal relations.
%	\item We propose an efficient temporal pattern mining method, HTPGM, that uses efficient data structures, \textit{bitmap} and Hierarchical Pattern Graph, to enable fast computations for support and confidence.
%	\item We propose two groups of pruning techniques based on the Apriori principle and the transitivity property of temporal events to enable faster mining. 
%	\item Based on mutual information, we derive the lower bound of confidence of temporal events, and based on that, to approximate HTPGM. This approximation can prune unpromising time series, and thus, significantly reduces the input size, allowing HTPGM scale on big datasets.
%	\item We perform extensive experiments on real-world datasets to show that HTPGM outperforms the baselines, with the approximate solution can achieve up to $3$ orders of magnitude speedup, consume less memory, and obtain high accuracy compared to the exact solution.
	
%\end{itemize}

%Temporal patterns can be mined upon specific times or with time intervals. The specific time-based approach is only efficient when handle instantaneous events not event intervals. Nonetheless, in reality, relations among events commonly happen at time intervals. TPM on time intervals have been investigated extensively, there are challenges. First, the complex interval-based relationships increase the candidates of temporal pattern generation, which leads to the high complexity of TPM.  Second, many uncorrelated temporal patterns are gained, which causes some difficulties in the final result analysis. Much of previous research of TPM are proposed. [ARMADA][ HDFS][ IEMiner] employ several optimization techniques to accelerate TPM process. [TPrefixSpan][ TPMiner][ TIEDSS] propose the temporal pattern representations, then develop the algorithms for TPM based on these representations. However, the complexity of relations among events and the uncorrelated temporal patterns generation still exist. 


==> MILowerBoundProof_Old.tex <==
\begin{proof} 

From Eq. \eqref{eq:NMI}, we have:
\begin{equation}
\small
\widetilde{I}(\mathcal{X}_S;\mathcal{Y}_S)= 1 - \frac{H(\mathcal{X}_S \vert \mathcal{Y}_S)}{H(\mathcal{X}_S)} \ge \mu
\end{equation} 
Hence:
\begin{equation}
\small
\frac{H(\mathcal{X}_S \vert \mathcal{Y}_S)}{H(\mathcal{X}_S)} \le  1-\mu
\label{eq:30}
\end{equation} 
First, we derive a lower bound for $\frac{H(\mathcal{X}_S \vert \mathcal{Y}_S)}{H(\mathcal{X}_S)}$.
\begin{align}
\small
\frac{H(\mathcal{X}_S \vert \mathcal{Y}_S)}{H(\mathcal{X}_S)} &= \frac{p(X_1, Y_1) \cdot \log p(X_1 \vert Y_1) }   {p(X_1) \cdot \log p(X_1) + \sum_{i \neq 1} p(X_i) \cdot \log p(X_i)} \nonumber \\ &+ \frac{\sum_{i \neq 1 \& j \neq 1} p(X_i, Y_j) \cdot \log \frac{p(X_i , Y_j)} {p(Y_j)}}{p(X_1) \cdot \log p(X_1) + \sum_{i \neq 1} p(X_i) \cdot \log p(X_i)}
\label{eq:31}
\end{align}			

Applying the log sum inequality \cite{thomas} for the second term of the denominator in Eq. \eqref{eq:31}, we get: 
\begin{align}
\small
\sum_{i \neq 1} p(X_i) \cdot \log p(X_i) &\geq \sum_{i \neq 1} p(X_i) \log\frac{\sum_{i \neq 1} p(X_i)}{\sum_{i \neq 1} 1} \\ &= (1-p(X_1)) \cdot \log\frac{1-p(X_1)}{n_x-1}
\label{eq:32}
\end{align}
\\	
Replace Eq. \eqref{eq:32} into Eq. \eqref{eq:31}, we get:
\begin{align}
\small
\frac{H(\mathcal{X}_S \vert \mathcal{Y}_S)}{H(\mathcal{X}_S)} \geq  \frac{p(X_1, Y_1) \cdot \log p(X_1 \vert Y_1)}{p(X_1) \cdot \log p(X_1) + (1-p(X_1)) \cdot \log\frac{1-p(X_1)}{n_x-1}} 
\label{eq:33}
\end{align}		
	
\textbf{$\ast$ Case 1:} Assuming that $\textit{supp}(Y_{1})_{\mathcal{D}_{\text{SYB}}} \ge \textit{supp}(X_{1})_{\mathcal{D}_{\text{SYB}}}$. Thus, the confidence of $(X_1,Y_1)$ in $\mathcal{D}_{\text{SYB}}$ is computed as
\begin{align}
\small
\textit{conf}(X_1,Y_1)_{\mathcal{D}_{\text{SYB}}} = \frac{\textit{supp}(X_1,Y_1)_{\mathcal{D}_{\text{SYB}}}}{\textit{supp}(Y_{1})_{\mathcal{D}_{\text{SYB}}}} = \frac{p(X_1,Y_1)}{p(Y_1)}
\end{align}	
%Since $(X_1, Y_1)$ is frequent in $\mathcal{D}_{S}$, we deduce $\sigma \leq supp(X_1,Y_1)_{\mathcal{D}_{Symbol}}=p(X_1, Y_1) \leq \sigma_m,  \sigma \leq supp(X_1)_{\mathcal{D}_{Symbol}}=p(X_1) \leq \sigma_m, \sigma \leq supp(Y_1)_{\mathcal{D}_{Symbol}}=p(Y_1) \leq \sigma_m$, it follows that: 
\\	
Since we have: $\log \frac{p(X_1,Y_1)}{p(Y_1)} < 0$, and $\sigma \le p(X_1,Y_1)$, we can deduce: 
\begin{equation}
\small
p(X_1,Y_1) \cdot \log \frac{p(X_1,Y_1)}{p(Y_1)} \leq \sigma \cdot \log \frac{p(X_1,Y_1)}{p(Y_1)}
\label{eq:case1_2}
\end{equation}
\\
We also have: $\log\sigma \leq \log p(X_1) <0$, and $p(X_1) \leq \sigma_m$, hence:
\begin{equation}
\small
p(X_1) \cdot \log p(X_1) \geq \sigma_m \cdot \log \sigma
\label{eq:case1_3}
\end{equation}
\\
We also get: $\log \frac{1-\sigma_m}{n_x - 1} \leq \log \frac{1-p(X_1)}{n_x-1} < 0$, and $(1-p(X_1)) \leq (1-\sigma)$, hence:
\begin{equation}
\small
(1-p(X_1)) \cdot \log \frac{1-p(X_1)}{n_x-1} \geq (1-\sigma) \cdot \log \frac{1-\sigma_m}{n_x - 1}
\label{eq:case1_4}
\end{equation}
 \\
From Eqs. \eqref{eq:case1_3}, \eqref{eq:case1_4}, we have: 
\begin{align}
\small
p(X_1) \cdot \log p(X_1) + (1-p(X_1)) \cdot \log\frac{1-p(X_1)}{n_x-1} \geq \nonumber &\\ \sigma_m \cdot \log \sigma + (1-\sigma) \cdot \log \frac{1-\sigma_m}{n_x - 1}
\label{eq:case1_5}
\end{align}
Replace Eq. \eqref{eq:case1_2} into the numerator, and Eq. \eqref{eq:case1_5} into the denominator of Eq. \eqref{eq:33}, we get:
\begin{align}
\small
\frac{H(\mathcal{X}_S \vert \mathcal{Y}_S)}{H(\mathcal{X}_S)} \geq \frac{\sigma \cdot \log \frac{p(X_1,Y_1)}{p(Y_1)}} {\sigma_m \cdot \log\sigma + (1-\sigma) \cdot \log\frac{1-\sigma_m}{n_x-1}} 
\label{eq:case1_6}
\end{align}			
\\	
From Eqs. \eqref{eq:30} and \eqref{eq:case1_6}, it follows that:
	\begin{align}
	\small
	(1-\mu) &\geq \frac{\sigma \cdot \log \frac{p(X_1,Y_1)}{p(Y_1)}} {\sigma_m \cdot \log\sigma + (1-\sigma) \cdot \log\frac{1-\sigma_m}{n_x-1}}  
	\label{eq:case1_7}
	\end{align}

	\begin{align}
	\small
	\Rightarrow \textit{conf}(X_1,Y_1)_{\mathcal{D}_{\text{SYB}}} &= \frac{p(X_1,Y_1)}{p(Y_1)} \\ &\geq \left(\sigma^{\sigma_m} \cdot \left(\frac{1-\sigma_m}{n_x-1}\right)^{1-\sigma} \right)^{\frac{1-\mu}{\sigma} } 
	\label{eq:case1_8}
	\end{align}
	
\textbf{$\ast$ Case 2:} Assuming that $\textit{supp}(Y_{1})_{\mathcal{D}_{\text{SYB}}} < \textit{supp}(X_{1})_{\mathcal{D}_{\text{SYB}}}$. Thus, the confidence of $(X_1,Y_1)$ in $\mathcal{D}_{\text{SYB}}$ is computed as 
\begin{equation}
\small
\textit{conf}(X_1,Y_1)_{\mathcal{D}_{\text{SYB}}} = \frac{p(X_1,Y_1)}{p(X_1)}
\label{eq:case2_1}
\end{equation}
From Eq. \eqref{eq:33}, we have:
	\begingroup
	\begin{align}
	\small
	\frac{H(\mathcal{X}_S \vert \mathcal{Y}_S)}{H(\mathcal{X}_S)} &\geq  \frac{p(X_1, Y_1) \cdot \log \left( \frac{p(X_1,Y_1)}{p(X_1)} \frac{p(X_1)}{p(Y_1)} \right)} {p(X_1) \cdot \log p(X_1) + (1-p(X_1)) \cdot \log\frac{1-p(X_1)}{n_x-1}} 	\label{eq:case2_2} \\
	&\geq \frac{\sigma \cdot \log \left( \frac{p(X_1,Y_1)}{p(X_1)} \cdot \frac{\sigma_m}{\sigma} \right) } {\sigma_m \cdot \log\sigma + (1-\sigma) \cdot \log\frac{1-\sigma_m}{n_x-1}} 
	\label{eq:case2_3}
	\end{align}
	\endgroup
From Eqs. \eqref{eq:30}, \eqref{eq:case2_3}, it follows that:
	\begin{align}
	\small
	 (1-\mu) &\geq \frac{\sigma \cdot \log \left( \frac{p(X_1,Y_1)}{p(X_1)} \cdot \frac{\sigma_m}{\sigma} \right) } {\sigma_m \cdot \log\sigma + (1-\sigma) \cdot \log\frac{1-\sigma_m}{n_x-1}}  
	 \label{eq:case2_4}
	\end{align}
	\begin{align}
	\small
	\Rightarrow \textit{conf}(X_1,Y_1)_{\mathcal{D}_{\text{SYB}}} &= \frac{p(X_1,Y_1)}{p(X_1)} \\ &\geq \left(\sigma^{\sigma_m} \cdot \left(\frac{1-\sigma_m}{n_x-1}\right)^{1-\sigma} \right)^{\frac{1-\mu}{\sigma} } \cdot \left(\frac{\sigma}{\sigma_m}\right) 
	\label{eq:case2_5}
	\end{align}
	\\
	In Eq. \eqref{eq:case2_5}, we have $\frac{\sigma}{\sigma_m} < 1$. Thus, from Eqs. \eqref{eq:case1_8}, \eqref{eq:case2_5}, we have the confidence lower bound of $(X_1,Y_1)$ in $\mathcal{D}_{\text{SYB}}$ in both cases is:
	\begingroup
	\begin{align}
	\small
	\textit{conf}(X_1,Y_1)_{\mathcal{D}_{\text{SYB}}}  &\geq  \left(\sigma^{\sigma_m} \cdot \left(\frac{1-\sigma_m}{n_x-1}\right)^{1-\sigma} \right)^{\frac{1-\mu}{\sigma} } 
	\label{eq:15}
	\end{align}
	\endgroup
	\\
	Next, we consider the confidence of $(X_1,Y_1)$ in the temporal sequence database $\mathcal{D}_{\text{SEQ}}$. From Lemma \ref{lem:supportconnection1}, we have:
	\begin{align}
	\small
	\textit{supp}(X_1)_{\mathcal{D}_{\text{SYB}}} \le \textit{supp}(X_1)_{\mathcal{D}_{\text{SEQ}}} \le \sigma_m
	\label{eq:confSeq1}
	\end{align}
	\begin{align}
	\small
	 \Rightarrow \textit{supp}(X_1)_{\mathcal{D}_{\text{SYB}}} + \beta_1 \le \sigma_m
	 \label{eq:confSeq2}
	\end{align}
	\begin{align}
	\small
	\Rightarrow \beta_1 \leq \sigma_m - \sigma
	\label{eq:confSeq3}
	\end{align}
	where $\beta_1$ is a non-negative number, and $\textit{supp}(X_1)_{\mathcal{D}_{\text{SYB}}} \ge \sigma$. 
	\\
	Without loss of generality, we assume that $\textit{supp}(X_1)_{\mathcal{D}_{\text{SEQ}}}$ $\ge$ $\textit{supp}(Y_1)_{\mathcal{D}_{\text{SEQ}}}$. Thus, the confidence of $(X_1,Y_1)$ in $\mathcal{D}_{\text{SEQ}}$ is computed as
	\begingroup
	\begin{align}
	\small
	\textit{conf}(X_1,Y_1)_{\mathcal{D}_{\text{SEQ}}} &=\frac{\textit{supp}(X_1,Y_1)_{\mathcal{D}_{\text{SEQ}}}}{\textit{supp}(X_1)_{\mathcal{D}_{\text{SEQ}}}} \geq \frac{\textit{supp}(X_1,Y_1)_{\mathcal{D}_{\text{SYB}}}}{\textit{supp}(X_1)_{\mathcal{D}_{\text{SYB}}}+\beta_2}
	\label{eq:confSeq4}
	\end{align}	
	From Eqs. \eqref{eq:confSeq3}, \eqref{eq:confSeq4}, we have:
	\begin{align}
	\small
	\textit{conf}(X_1,Y_1)_{\mathcal{D}_{\text{SEQ}}} \geq \frac{\textit{supp}(X_1,Y_1)_{\mathcal{D}_{\text{SYB}}}} {\textit{supp}(X_1)_{\mathcal{D}_{\text{SYB}}}+\sigma_m - \sigma} 
	\label{eq:12}
	\end{align}
	\endgroup
	\\
From Eq. \ref{eq:15}, we get:
\begin{align}
\small
\textit{conf}(X_1,Y_1)_{\mathcal{D}_{\text{SYB}}} &= \frac{\textit{supp}(X_1,Y_1)_{\mathcal{D}_{\text{SYB}}}}{supp(X_1)_{\mathcal{D}_{\text{SYB}}}} \nonumber \\ &\geq \left(\sigma^{\sigma_m} \cdot \left(\frac{1-\sigma_m}{n_x-1}\right)^{1-\sigma} \right)^{\frac{1-\mu}{\sigma} } 
\label{eq:confSeq5}
\end{align}
Let:
\begin{equation}
\small
l= \left(\sigma^{\sigma_m} \cdot \left(\frac{1-\sigma_m}{n_x-1}\right)^{1-\sigma} \right)^{\frac{1-\mu}{\sigma}} 
\label{eq:confSeq6}
\end{equation}
From Eqs. \eqref{eq:12}, \eqref{eq:confSeq5}, \eqref{eq:confSeq6}, we have:
\begin{align}
 \frac{supp(X_1,Y_1)_{\mathcal{D}_{\text{SYB}}}} {supp(X_1)_{\mathcal{D}_{\text{SYB}}}+\sigma_m - \sigma} &\geq \frac{l \cdot supp(X_1)_{\mathcal{D}_{\text{SYB}}}}{supp(X_1)_{\mathcal{D}_{\text{SYB}}}+\sigma_m - \sigma}  \\
&\geq \frac{l \cdot \sigma}{\sigma_m + \sigma_m - \sigma} = \frac{l \cdot \sigma}{2 \cdot \sigma_m - \sigma} \label{eq:16}
\end{align}
Finally, from Eqs. \eqref{eq:12} and \eqref{eq:16}, we can conclude:
\resizebox{1\columnwidth}{!}{
	\begin{minipage}{\columnwidth}
		\begingroup
		\begin{align}
		\textit{conf}(X_1,Y_1)_{\mathcal{D}_{\text{SEQ}}}  &\geq  \left(\sigma^{\sigma_m} \cdot \left(\frac{1-\sigma_m}{n_x-1}\right)^{1-\sigma} \right)^{\frac{1-\mu}{\sigma} } \cdot \frac{\sigma}{2 \cdot \sigma_m - \sigma} \nonumber
		\end{align}
		\endgroup
	\end{minipage}
}
\end{proof}

==> MIProof.tex <==
\begin{proof}
	We denote support and all-confidence of $(X_1,Y_1)$ in $\mathcal{D}_{S}$ as $supp(X_1,Y_1)_{\mathcal{D}_{S}}$ and $\textit{all-conf}(X_1,Y_1)_{\mathcal{D}_{S}}$, and support and all-confidence of $(X_1,Y_1)$ in $\mathcal{D}_{Symbol}$ as $supp(X_1,Y_1)_{\mathcal{D}_{Symbol}}$ and $\textit{all-conf}(X_1,Y_1)_{\mathcal{D}_{Symbol}}$. 
	
	Since $(X_1$, $Y_1)$ is a pair of frequent temporal events in $\mathcal{D}_{S}$, hence  $\sigma \leq supp(X_1,Y_1)_{\mathcal{D}_{S}} \leq \sigma_m$.
	Now we prove that if $\sigma \leq supp(X_1,Y_1)_{\mathcal{D}_{Symbol}} \leq \sigma_m$ then $\sigma \leq supp(X_1,Y_1)_{\mathcal{D}_{S}} \leq \sigma_m$.
	
	We have: $supp(X_1,Y_1)_{D_{Symbol}} = \frac{\sum_{i=1}^{n/m} a_i} {n}$; where $x_i$ is the number of occurrence of $(X_1,Y_1)$ in duration $T_i+t_{max}$, $n$ is the number of transactions in $\mathcal{D}_{Symbol}$, $m$ is the number of granularity units of each $T_i+t_{max}$. In $\mathcal{D}_S$, the support of $X_1$ and $Y_1$ is calculated as follows. If $(X_1,Y_1)$ occurs many times at $T_i+t_{max}$ in $\mathcal{D}_{Symbol}$, we consider (X,Y) only occurs once equivalent with $T_i+t_{max}$ in $\mathcal{D}_S$. We deduce: 
	
	$supp(X_1,Y_1)_{D_S} = \frac{\sum_{i=1}^{n/m} b_i} {n/m} = \frac{m \cdot \sum_{i=1}^{n/m} b_i} {n} $,
	where 
	\[b_i = \begin{cases}
	1,& \text{if } (a_i \text{ in } \mathcal{D}_{Symbol}) > 0\\
	0,              & \text{otherwise}
	\end{cases}\]
	
	Since $a_i \leq m \cdot b_i$ $(1 \leq i \leq n/m)$, hence $supp(X_1,Y_1)_{D_{Symbol}} \leq supp(X_1,Y_1)_{D_S}$. So $\sigma \leq supp(X_1,Y_1)_{D_{Symbol}} \leq \sigma_m$, then $\sigma \leq supp(X_1,Y_1)_{D_S} \leq \sigma_m$.
	
	Now we infer upper and lower bounds of $\textit{all-conf}(X_1,Y_1)_{\mathcal{D}_{S}}$. Without loss of generality, we assume that $\textit{all-conf}(X_1,Y_1)_{D_S} = \frac{supp(X_1,Y_1)_{D_S}}{supp(X_1)_{D_S}}$. 
	We have:
	\resizebox{1\columnwidth}{!}{
		\begin{minipage}{\columnwidth}
			\begin{align}
			&supp(X_1,Y_1)_{D_S} = supp(X_1,Y_1)_{D_{Symbol}} + \beta_1 \leq \sigma_m  \Rightarrow \beta_1 \leq \sigma_m - \sigma \nonumber\\
			&supp(X_1)_{D_S} = supp(X_1)_{D_{Symbol}} + \beta_2 \leq \sigma_m 
			\Rightarrow \beta_2 \leq \sigma_m - \sigma \nonumber
			\end{align}
		\end{minipage}
	}
	
	We deduce an upper bound of $\textit{all-conf}(X_1,Y_1)_{\mathcal{D}_{S}}$:
	
	\resizebox{.97\columnwidth}{!}{
		\begin{minipage}{\columnwidth}
			\begingroup
			\small
			\begin{align}
			&\frac{supp(X_1,Y_1)_{D_S}}{supp(X_1)_{D_S}} \leq \frac{supp(X_1,Y_1)_{D_{Symbol}} +\beta_1}{supp(X_1)_{D_{Symbol}}} \nonumber\\
			\Rightarrow & \textit{all-conf}(X_1,Y_1)_{D_S} \leq \frac{supp(X_1,Y_1)_{D_{Symbol}} + \sigma_m - \sigma}{supp(X_1)_{D_{Symbol}}} \label{eq:11}
			\end{align}
			\endgroup
		\end{minipage}
	}
	
	We also deduce a lower bound of $\textit{all-conf}(X_1,Y_1)_{\mathcal{D}_{S}}$:
	\resizebox{1\columnwidth}{!}{
		\begin{minipage}{\columnwidth}
			\begingroup
			\small
			\begin{align}
			&\frac{supp(X_1,Y_1)_{D_S}}{supp(X_1)_{D_S}} \geq \frac{supp(X_1,Y_1)_{D_{Symbol}}}{supp(X_1)_{D_{Symbol}}+\beta_2} \nonumber\\
			\Rightarrow & \textit{all-conf}(X_1,Y_1)_{D_S} \geq \frac{supp(X_1,Y_1)_{D_{Symbol}}} {supp(X_1)_{D_{Symbol}}+\sigma_m - \sigma} \label{eq:12}
			\end{align}
			\endgroup
		\end{minipage}
	}
	
	To prove part (a), we show that if $\widetilde{I}(X, Y) < \mu$, $\textit{all-conf}(X_1,Y_1)_{\mathcal{D}_{S}}$ has an upper bound. We have $\widetilde{I}(X, Y)= 1 - \frac{H(X \vert Y)}{H(X)} < \mu$, hence $\frac{H(X \vert Y)}{H(X)} > 1-\mu$. Now we derive an upper bound for $\frac{H(X \vert Y)}{H(X)}$. Observe that $\widetilde{I}(X, Y)$ is calculated on $\mathcal{D}_{Symbol}$, hence:
	\resizebox{1\columnwidth}{!}{
		\begin{minipage}{\columnwidth}
			\begingroup
			\small
			\begin{align}
			&\frac{H(X \vert Y)}{H(X)} = \frac{-\sum_{i=1}^{n_x} \sum_{j=1}^{n_y} p(X_i, Y_j) \cdot \log p(X_i \vert Y_j) }   {-\sum_{i=1}^{n_x} p(X_i) \cdot \log p(X_i)} = \nonumber\\
			&\frac{p(X_1, Y_1) \cdot \log p(X_1 \vert Y_1) +\sum_{i \neq 1 \& j \neq 1} p(X_i, Y_j) \cdot \log \frac{p(X_i , Y_j)} {p(Y_j)} }   {p(X_1) \cdot \log p(X_1) + \sum_{i \neq 1}^{n_x} p(X_i) \cdot \log p(X_i)} \label{eq:13}
			\end{align}
			\endgroup
		\end{minipage}
	}
	
	By applying the log sum inequality for the second term in the numerator of equation (\ref{eq:13}), we get: 
	
	\begin{equation}
	\small
	\sum\nolimits_{i \neq 1 \& j \neq 1} p(X_i, Y_j) \cdot \log \frac{p(X_i , Y_j)} {p(Y_j)} \geq \sum\nolimits_{i \neq 1 \& j \neq 1} p(X_i, Y_j) \cdot \log \frac{\sum\nolimits_{i \neq 1 \& j \neq 1} p(X_i, Y_j)} {\sum\nolimits_{i \neq 1 \& j \neq 1} p(Y_j)} = \left(1-p(X_1, Y_1)\right) \cdot \log \frac{1-p(X_1, Y_1)}{n_x - p(Y_1)}
	\end{equation}
	
	Consider the second term in the denominator of equation (\ref{eq:13}), we get: 
	\begin{equation}
	\small
	\sum_{i \neq 1}^{n_x} p(X_i) \cdot \log p(X_i) \leq (1-p(X_1) \cdot \log (1-P(X_1))
	\end{equation}
	
	
	Finally, we deduce that:
	
	\resizebox{1\columnwidth}{!}{
		\begin{minipage}{\columnwidth}
			\begin{align}
			\frac{H(X \vert Y)}{H(X)} \leq \frac{p(X_1, Y_1) \cdot \log p(X_1 \vert Y_1) + \left(1-p(X_1, Y_1)\right) \cdot \log \frac{1-p(X_1, Y_1)}{n_x - p(Y_1)}} {p(X_1) \cdot \log p(X_1) + (1-p(X_1)) \cdot \log (1-p(X_1)) } \nonumber
			\end{align}
		\end{minipage}
	}
	
	We have: $\textit{all-conf}(X_1,Y_1)_{\mathcal{D}_{Symbol}} = \frac{p(X_1,Y_1)}{max\{p(X_1),p(Y_1)\}}$.
	
	$\textbf{Case a\textsubscript{1}:} {\textit{ all-conf}(X_1,Y_1)_{\mathcal{D}_{Symbol}} = \frac{p(X_1,Y_1)}{p(Y_1)}}$
	\resizebox{1\columnwidth}{!}{
		\begin{minipage}{\columnwidth}
			\begin{align}
			\frac{H(X \vert Y)}{H(X)} &\leq \frac{p(X_1, Y_1) \cdot \log \frac{p(X_1,Y_1)}{p(Y_1)} + \left(1-p(X_1, Y_1)\right) \cdot \log \frac{1-p(X_1, Y_1)}{n_x - p(Y_1)}} {p(X_1) \cdot \log p(X_1) + \log (1-p(X_1)) \cdot (1-p(X_1))}  \nonumber
			\end{align}
		\end{minipage}
	}
	
	Since $(X_1, Y_1)$ is frequent in $\mathcal{D}_{S}$, we deduce $\sigma \leq supp(X_1,Y_1)_{\mathcal{D}_{Symbol}}=p(X_1, Y_1) \leq \sigma_m,  \sigma \leq supp(X_1)_{\mathcal{D}_{Symbol}}=p(X_1) \leq \sigma_m, \sigma \leq supp(Y_1)_{\mathcal{D}_{Symbol}}=p(Y_1) \leq \sigma_m$, it follows that: 
	
	\resizebox{1\columnwidth}{!}{
		\begin{minipage}{\columnwidth}
			\begin{align}
			&& \frac{H(X \vert Y)}{H(X)} &\leq \frac{\sigma_m \cdot \log \frac{p(X_1,Y_1)}{p(Y_1)} + (1-\sigma) \cdot \log \frac{1-\sigma_m}{n_x-\sigma}}{\sigma \cdot \log \sigma_m + (1-\sigma_m) \cdot \log (1-\sigma)} \nonumber\\
			& \Rightarrow &(1-\mu) &< \frac{\sigma_m \cdot \log \frac{p(X_1,Y_1)}{p(Y_1)} + (1-\sigma) \cdot \log \frac{1-\sigma_m}{n_x-\sigma}}{\sigma \cdot \log \sigma_m + (1-\sigma_m) \cdot \log (1-\sigma)} \nonumber\\
			& \Leftrightarrow &\frac{p(X_1,Y_1)}{p(Y_1)} &< \left( \left(\sigma_{m}^{\sigma} \cdot (1-\sigma)^{1-\sigma_m} \right)^{1-\mu} \cdot \left(\frac{n_x-\sigma}{1-\sigma_m}\right)^{1-\sigma} \right)^{{\frac{1}{\sigma_m}}} \nonumber
			\end{align}
		\end{minipage}
	}
	
	\textbf{Case a\textsubscript{2}:} $\textit{all-conf}(X_1,Y_1)_{\mathcal{D}_{Symbol}} = \frac{p(X_1,Y_1)}{p(X_1)}$
	
	\resizebox{1\columnwidth}{!}{
		\begin{minipage}{\columnwidth}
			\begin{align}
			\frac{H(X \vert Y)}{H(X)} &\leq \frac{p(X_1, Y_1) \cdot \log \left( \frac{p(X_1,Y_1)}{p(X_1)} \cdot \frac{p(X_1)}{p(Y_1)} \right) + \left(1-p(X_1, Y_1)\right) \cdot \log \frac{1-p(X_1, Y_1)}{n_x - p(Y_1)}} {p(X_1) \cdot \log p(X_1) + \log (1-p(X_1)) \cdot (1-p(X_1))}  \nonumber\\
			&\leq \frac{\sigma_m \cdot \log \left( \frac{p(X_1,Y_1)}{p(X_1)} \cdot \frac{\sigma}{\sigma_m} \right) + (1-\sigma) \cdot \log \frac{1-\sigma_m}{n_x-\sigma}}{\sigma \cdot \log \sigma_m + (1-\sigma_m) \cdot \log (1-\sigma)} \nonumber
			\end{align}
		\end{minipage}
	}
	
	\resizebox{1\columnwidth}{!}{
		\begin{minipage}{\columnwidth}
			\begin{align}
			&\Rightarrow &(1-\mu) &< \frac{\sigma_m \cdot \log \left( \frac{p(X_1,Y_1)}{p(X_1)} \cdot \frac{\sigma}{\sigma_m} \right) + (1-\sigma) \cdot \log \frac{1-\sigma_m}{n_x-\sigma}}{\sigma \cdot \log \sigma_m + (1-\sigma_m) \cdot \log (1-\sigma)} \nonumber\\
			&\Leftrightarrow &\frac{p(X_1,Y_1)}{p(X_1)} &< \left( 
			\left(\sigma_{m}^{\sigma} \cdot (1-\sigma)^{1-\sigma_m} \right)^{1-\mu} \cdot \left(\frac{n_x-\sigma}{1-\sigma_m}\right)^{1-\sigma} 
			\right)^{\frac{1}{\sigma_m}} \cdot \frac{\sigma_m}{\sigma} \nonumber
			\end{align}
		\end{minipage}
	}
	
	Now, we consider the upper bound of all-confidence in both of two cases. Since $\frac{\sigma_m}{\sigma} >1$, thus we have:
	\resizebox{.95\columnwidth}{!}{
		\begin{minipage}{\columnwidth}
			\begingroup
			\footnotesize
			\begin{align}
			\textit{all-conf}(X_1,Y_1)_{\mathcal{D}_{Symbol}} < \left( \left(\sigma_{m}^{\sigma} \cdot (1-\sigma)^{1-\sigma_m} \right)^{1-\mu} \cdot \left(\frac{n_x-\sigma}{1-\sigma_m}\right)^{1-\sigma} \right)^{{\frac{1}{\sigma_m}}} \label{eq:14}
			\end{align}
			\endgroup
		\end{minipage}
	}
	
	From two equations (\ref{eq:11}) and (\ref{eq:14}), we have the conclusion:
	\resizebox{1\columnwidth}{!}{
		\begin{minipage}{\columnwidth}
			\begin{align}
			\textit{all-conf}(X_1,Y_1)_{\mathcal{D}_S} < \left( \left(\sigma_{m}^{\sigma} \cdot (1-\sigma)^{1-\sigma_m} \right)^{1-\mu} \cdot \left(\frac{n_x-\sigma}{1-\sigma_m}\right)^{1-\sigma} \right)^{{\frac{1}{\sigma_m}}} + \frac{\sigma_m -\sigma}{\sigma} 
			\end{align}
		\end{minipage}
	}
	\\In order to prove part (b), we show if $\widetilde{\mathit{I}}(X, Y) \geq \mu$, $\textit{all-conf}(X_1,Y_1)_{\mathcal{D}_{S}}$ has a lower bound. First, we derive a lower bound for $\frac{H(X \vert Y)}{H(X)}$.
	\resizebox{1\columnwidth}{!}{
		\begin{minipage}{\columnwidth}
			\begingroup
			\begin{align}
			\frac{H(X \vert Y)}{H(X)} &= \frac{p(X_1, Y_1) \cdot \log p(X_1 \vert Y_1) + \sum_{i \neq 1 \& j \neq 1} p(X_i, Y_j) \cdot \log \frac{p(X_i , Y_j)} {p(Y_j)} }   {p(X_1) \cdot \log p(X_1) + \sum_{i \neq 1} p(X_i) \cdot p(X_i)} \nonumber \\
			&\geq  \frac{p(X_1, Y_1) \cdot \log p(X_1 \vert Y_1)}{p(X_1) \cdot \log p(X_1) + (1-p(X_1)) \cdot \log\frac{1-p(X_1)}{n_x-1}} 
			\end{align}
			\endgroup  
		\end{minipage}
	}
	$\textbf{Case b\textsubscript{1}:} {\textit{ all-conf}(X_1,Y_1)_{\mathcal{D}_{Symbol}} = \frac{p(X_1,Y_1)}{p(Y_1)}}$
	\resizebox{1\columnwidth}{!}{
		\begin{minipage}{\columnwidth}
			\begin{align}
			\frac{H(X \vert Y)}{H(X)} &\geq  \frac{p(X_1, Y_1) \cdot \log \frac{p(X_1,Y_1)}{p(Y_1)}}{p(X_1) \cdot \log p(X_1) + (1-p(X_1)) \cdot \log\frac{1-p(X_1)}{n_x-1}}  \nonumber\\
			&\geq \frac{\sigma \cdot \log \frac{p(X_1,Y_1)}{p(Y_1)}} {\sigma_m \cdot \log\sigma + (1-\sigma) \cdot \log\frac{1-\sigma_m}{n_x-1}} 
			\end{align}
		\end{minipage}
	}
	
	Since $\frac{H(X \vert Y)}{H(X)} \leq (1-\mu)$, it follows that:
	\begingroup
	\begin{align}
	(1-\mu) &\geq \frac{\sigma \cdot \log \frac{p(X_1,Y_1)}{p(Y_1)}} {\sigma_m \cdot \log\sigma + (1-\sigma) \cdot \log\frac{1-\sigma_m}{n_x-1}} \nonumber \\
	\Leftrightarrow \frac{p(X_1,Y_1)}{p(Y_1)} &\geq \left(\sigma^{\sigma_m} \cdot \left(\frac{1-\sigma_m}{n_x-1}\right)^{1-\sigma} \right)^{\frac{1-\mu}{\sigma} } 
	\end{align}
	\endgroup
	
	\textbf{Case b\textsubscript{2}:} $\textit{all-conf}(X_1,Y_1)_{\mathcal{D}_{Symbol}} = \frac{p(X_1,Y_1)}{p(X_1)}$
	\begingroup
	\begin{align}
	\frac{H(X \vert Y)}{H(X)} &\geq  \frac{p(X_1, Y_1) \cdot \log \left( \frac{p(X_1,Y_1)}{p(X_1)} \frac{p(X_1)}{p(Y_1)} \right)} {p(X_1) \cdot \log p(X_1) + (1-p(X_1)) \cdot \log\frac{1-p(X_1)}{n_x-1}}  \nonumber\\
	&\geq \frac{\sigma \cdot \log \left( \frac{p(X_1,Y_1)}{p(X_1)} \cdot \frac{\sigma_m}{\sigma} \right) } {\sigma_m \cdot \log\sigma + (1-\sigma) \cdot \log\frac{1-\sigma_m}{n_x-1}} 
	\end{align}
	\endgroup
	
	\begingroup
	\begin{align}
	\Rightarrow (1-\mu) &\geq \frac{\sigma \cdot \log \left( \frac{p(X_1,Y_1)}{p(X_1)} \cdot \frac{\sigma_m}{\sigma} \right) } {\sigma_m \cdot \log\sigma + (1-\sigma) \cdot \log\frac{1-\sigma_m}{n_x-1}} \nonumber \\
	\Leftrightarrow \frac{p(X_1,Y_1)}{p(X_1)} &\geq \left(\sigma^{\sigma_m} \cdot \left(\frac{1-\sigma_m}{n_x-1}\right)^{1-\sigma} \right)^{\frac{1-\mu}{\sigma} } \cdot \left(\frac{\sigma}{\sigma_m}\right) 
	\end{align}
	\endgroup
	
	Now, we consider the lower bound of all-confidence in both of two cases. Since $\frac{\sigma}{\sigma_m} <1$, thus 
	\iffalse
	\begingroup
	\scriptsize
	\begin{align}
	\left(\sigma^{\sigma_m} \cdot \left(\frac{1-\sigma_m}{n_x-1}\right)^{1-\sigma} \right)^{\frac{1-\mu}{\sigma} } \cdot \left(\frac{\sigma}{\sigma_m}\right) <  \left(\sigma^{\sigma_m} \cdot \left(\frac{1-\sigma_m}{n_x-1}\right)^{1-\sigma} \right)^{\frac{1-\mu}{\sigma} } 
	\end{align}
	\endgroup
	\fi
	we have:
	\begingroup
	\begin{align}
	\textit{all-conf}(X_1,Y_1)_{\mathcal{D}_{Symbol}}  &\geq  \left(\sigma^{\sigma_m} \cdot \left(\frac{1-\sigma_m}{n_x-1}\right)^{1-\sigma} \right)^{\frac{1-\mu}{\sigma} } 
	\label{eq:15}
	\end{align}
	\endgroup
	
	From two equations (\ref{eq:12}) and (\ref{eq:15}), we have the conclusion:
	\resizebox{1\columnwidth}{!}{
		\begin{minipage}{\columnwidth}
			\begingroup
			\begin{align}
			\textit{all-conf}(X_1,Y_1)_{\mathcal{D}_S}  &\geq  \left(\sigma^{\sigma_m} \cdot \left(\frac{1-\sigma_m}{n_x-1}\right)^{1-\sigma} \right)^{\frac{1-\mu}{\sigma} } \cdot \frac{\sigma}{2 \cdot \sigma_m - \sigma} 
			\end{align}
			\endgroup
		\end{minipage}
	}
\end{proof}

==> NewMethodBk.tex <==
\subsection{New method}


\hspace{-0.15in}\textbf{Property 3.4} Given a pattern $P$, if there exist two events, $E_i$ and $E_j$ are in $P$, such that $\frac{supp(E_i)}{supp(E_j)} \leq \delta$ then \textit{conf($P$)} $\leq \delta$.
\iffalse
\begin{proof}
	\begin{equation}
	\small
	\text{\it{conf(P)}} = \frac{supp(P)}{\max_{1 \leq k \leq n}\{supp(E_k) \}} \leq \frac{supp(E_i)}{\max_{1 \leq k \leq n}\{supp(E_k) \}} \leq \frac{supp(E_i)}{supp(E_j)} \leq \delta
	\end{equation}
\end{proof}
\fi

\hspace{-0.15in}\textbf{Property 3.5} (Cross-support property of confidence \cite{ke2008correlated}) Given a pattern $P$, if there exist a sub-pattern $P_X \in P$ , such that $\frac{supp(P_X)}{\max_{1 \leq k \leq n}\{supp(E_k) \}} \leq \delta$ (where $n$ is size of $P$ and $E_k$ is a temporal event in $P$) then \textit{conf($P$)} $\leq \delta$.
\iffalse
\begin{proof}
	\begin{equation}
	\small
	\text{\it{conf(P)}} = \frac{supp(P)}{\max_{1 \leq k \leq n}\{supp(E_k) \}} \leq \frac{supp(P_X)}{\max_{1 \leq k \leq n}\{supp(E_k) \}} \leq \delta
	\end{equation}
\end{proof}
\fi
In this section, we present a proposed algorithm, called Optimized Correlated Temporal Pattern Mining (OpCTPM) for the CTPM problem.
The OpCTPM uses three optimization techniques. The first technique is that we apply Apriori pruning principle. The second technique is to use the properties 4.3 and 4.4 of all-confidence. The first two techniques eliminate the redundant operations of finding the correlated temporal patterns. Finally, we use lemmas of temporal relations which are proved in the following section. This technique assists in finding out the relations among temporal events quickly.

\hspace{-0.15in}\textbf{Lemma 2:} The three temporal relations are mutual exclusive.
\begin{proof} Let two temporal events $E_1$ and $E_2$, and their corresponding instances, $e_1$ occurring during $[t_{s_1}, t_{e_1}]$ and $e_2$ occurring during $[t_{s_2}, t_{e_2}]$.
	There are three temporal relations that can happen between $E_1$ and $E_2$. Now we prove that if one of three relations happens then the remaining two relations do not happen. We consider the following cases.
	
	\hspace{-0.15in}\textit{Case 1:} We assume Follows($E_{1_{\triangleright e_1}}$, $E_{2_{\triangleright e_2}}$).
	
	\hspace{-0.15in}\textit{i.} We prove that Contains($E_{1_{\triangleright e_1}}$, $E_{2_{\triangleright e_2}}$) does not exist and vice versa.
	
	We have: Follows($E_{1_{\triangleright e_1}}$, $E_{2_{\triangleright e_2}})  \Rightarrow t_{e_1} \pm \epsilon \leq t_{s_2} $. 
	We also get: $t_{s_2} < t_{e_2}$.
	It follows: $t_{e_1} \pm \epsilon <  t_{e_2}$, and hence Contains($E_{1_{\triangleright e_1}}$, $E_{2_{\triangleright e_2}}$) condition is not satisfied $(t_{e_1} \pm \epsilon \geq  t_{e_2})$. Contrarily, Contains($E_{1_{\triangleright e_1}}$, $E_{2_{\triangleright e_2}}$) happens then Follows($E_{1_{\triangleright e_1}}$, $E_{2_{\triangleright e_2}}$) does not exist.
	
	\hspace{-0.15in}\textit{ii.} We prove that Overlaps($E_{1_{\triangleright e_1}}$, $E_{2_{\triangleright e_2}}$) does not exist and vice versa.
	
	We have: Follows($E_{1_{\triangleright e_1}}$, $E_{2_{\triangleright e_2}})  \Rightarrow t_{e_1} - t_{s_2} \leq \pm \epsilon$, thus Overlaps($E_{1_{\triangleright e_1}}$, $E_{2_{\triangleright e_2}}$) condition is not satisfied $(t_{e_1} - t_{s_2} \geq d_o \pm \epsilon)$. Contrarily, Overlaps($E_{1_{\triangleright e_1}}$, $E_{2_{\triangleright e_2}}$) happens then Follows($E_{1_{\triangleright e_1}}$, $E_{2_{\triangleright e_2}}$) does not exist.
	
	\hspace{-0.15in}\textit{Case 2:} We assume Contains($E_{1_{\triangleright e_1}}$, $E_{2_{\triangleright e_2}}$).
	
	We have: Contains$(E_{1_{\triangleright e_1}}$, $E_{2_{\triangleright e_2}}) \Rightarrow t_{e_1} \pm \epsilon \geq t_{e_2}$, thus Overlaps($E_{1_{\triangleright e_1}}$, $E_{2_{\triangleright e_2}}$) condition is not satisfied $(t_{e_1} \pm \epsilon < t_{e_2})$. Contrarily, Overlaps($E_{1_{\triangleright e_1}}$, $E_{2_{\triangleright e_2}}$) happens then Contains($E_{1_{\triangleright e_1}}$, $E_{2_{\triangleright e_2}}$) does not exist.
\end{proof}

\hspace{-0.15in}\textbf{Lemma 3:} Let $\Re$ = \{Follow, Contain, Overlap\} be a set of relations and $I_E$ be a set of temporal events. $\Re$ is transitive on $I_E$.

$ E_1, E_2, E_3 \in I_E; r_1, r_2 \in \Re: (r_1$ holds between $E_{1_{\triangleright e_1}}$  and  $E_{2_{\triangleright e_2}} ) \wedge (r_2$ holds between $E_{2_{\triangleright e_2}}$ and  $E_{3_{\triangleright e_3}} ) \Rightarrow \exists r_3 \in \Re \wedge (r_3$ holds between $E_{1_{\triangleright e_1}}$ and  $E_{3_{\triangleright e_3}} )$.

\begin{proof}
	Let three temporal events $E_1$, $E_2$, $E_3$, and their corresponding instance, $e_1$ occurring during $[t_{s_1}, t_{e_1}]$, $e_2$ occurring during $[t_{s_2}, t_{e_2}]$, and $e_3$ occurring during $[t_{s_3}, t_{e_3}]$. 
	
	First, we show that $\forall r \in \Re: r$ holds between $E_{1_{\triangleright e_1}}$ and  $E_{2_{\triangleright e_2}} \Rightarrow t_{s_1} \leq t_{s_2}$.
	
	\begin{itemize}
		\item Consider r = ``Follow", then: $t_{e_1} \pm \epsilon \leq t_{s_2} \Rightarrow t_{e_1} \leq t_{s_2} \pm \epsilon$.
		We always get: $\epsilon < t_{e_1} - t_{s_1} \Rightarrow t_{e_1} > t_{s_1} + \epsilon$.
		Thus: $t_{s_1} + \epsilon < t_{s_2} \pm \epsilon \Rightarrow t_{s_1} < t_{s_2}$.
		\item Consider r = ``Contain": from the definition of Contains($E_{1_{\triangleright e_1}}, E_{2_{\triangleright e_2}}$) relation, we have $t_{s_1} \leq t_{s_2}$.
		\item Consider r = ``Overlap": from the definition of Overlaps($E_{1_{\triangleright e_1}}, E_{2_{\triangleright e_2}}$) relation, we have $t_{s_1} < t_{s_2}$.
	\end{itemize}
	
	Thus, we conclude: $\forall r \in \Re: r$ holds between $E_{1_{\triangleright e_1}}$ and  $E_{2_{\triangleright e_2}} \Rightarrow t_{s_1} \leq t_{s_2}$.
	
	We have: $r_1 \in \Re$, $r_1$ holds between $E_{1_{\triangleright e_1}}$ and  $E_{2_{\triangleright e_2}} \Rightarrow t_{s_1} \leq t_{s_2}$; $r_2 \in \Re$, $r_2$ holds between $E_{2_{\triangleright e_2}}$ and  $E_{3_{\triangleright e_3}} \Rightarrow t_{s_2} \leq t_{s_3}$. It follows: $t_{s_1} \leq t_{s_3}$, thus we conclude: it exists a relation between $E_1$ and $E_3$, i.e. $\exists r_3 \in \Re: r_3$ holds between $E_{1_{\triangleright e_1}}$ and  $E_{3_{\triangleright e_3}}$.
\end{proof}

\subsubsection{Patterns enumeration tree}
In the next section, we use a tree-based structure to describe the process of the CTPM, which is called the \textit{patterns enumeration tree}. The tree's structure is as follows. The root of tree is an empty set. Each level k consists of a set of nodes, denoted as N(k), that hold the set of k-event patterns. Let $n^k_i$ denote $i^{th}$ node at level k. Every node $n^k_i$ holds a set of labels $\Sigma$ and a set of \textit{pattern nodes} $P^k(n^k_i)$. $\Sigma$ contains names of events and is used to generate patterns. Each $P^k(n^k_i)$ represents k-event patterns which is formed by the events in node $n^k_i$.

Furthermore, to accelerate mining process, we use TIID (Time Interval Identifier) structure as a compact representation of a \textit{pattern node} in the patterns enumeration tree. A TIID represents time interval in which a temporal pattern occurs. Each row in the TIID is a tuple $(id, \textit{TI-Set})$, where $id$ is a temporal sequence id in $\mathcal{D}_S$ and \textit{TI-Set} is a set of time intervals which the temporal pattern occurs at $id$. 

\textbf{Example 4.} Fig. \ref{fig:patternTree} is an example of a patterns enumeration tree. At level 1, $N(1)$=\{A[ON], A[OFF], B[ON], B[OFF], C[ON], C[OFF], D[OFF]\}. Level 1 is a special case in which each node $n^1_k$ is also a \textit{pattern node} $P^1(n^1_k)$. Each node at level 1 has a TIID. For example, the TIID of node ``A[ON]" occurs at $ids = \{1, 2, 3, 4\}$ along with the time intervals, respectively. At level 2, each node composes $\Sigma$ containing names of two events and the \textit{pattern nodes} of 2-event patterns. For instance, node ``A[ON], B[ON]" composes $\Sigma = $ \{A[ON], B[ON]\} and one pattern node ``A[ON] $\succcurlyeq$ B[ON]"; besides, the pattern node ``A[ON] $\succcurlyeq$ B[ON]" also has a TIID.
\begin{figure*}[h!]
	\centering
	\includegraphics[width=\textwidth, height=10.00cm]{figures/PatternTree.pdf}
	\caption{A patterns enumeration tree}
	\label{fig:patternTree}
\end{figure*}

To assist in support counting, we introduce a \textit{bitmap b} for each node (composing pattern node) to track temporal sequences ids in which the node occurs. Each \textit{bitmap b} has length $|\mathcal{D}_S|$, and each element \textit{b[i]} is 1 or 0, indicating whether the event or the pattern is present in row \textit{i} of $\mathcal{D}_S$ or not. To compute support value among two events or two patterns, we perform a logic AND operation on their bitmaps and count the number of values 1 on the bitmap.
\subsubsection{Mining process}
Algorithm \ref{algorithmOpTPM} illustrates the mining process to build the patterns enumeration tree. First, database $\mathcal{D}_S$ is converted from $\mathcal{D}_T$ (line 1). Consequently, we search for the set of frequent single events at level 1 (lines 2-6). We compute the support value of every event \textit{e} in $\mathcal{D}_{S}$. If \textit{rel-supp}(\textit{e}) $>\sigma$ then \textit{e} is added to level 1 and its TIID and bitmap are also updated respectively.

To mine the correlated 2-event patterns, we use the frequent single events at level 1. In this step, we apply two techniques for optimization of finding the correlated patterns. The first technique is based on \textit{Apriori principle}: let $p$ be a 2-event pattern that is frequent in $\mathcal{D}_{S}$, two events that form $p$ must be at least $\sigma$. The second technique is to apply the \textit{property 4.3} of the all-confidence: if the support ratio of two events is less than $\delta$ then the all-confidence of 2-event pattern which is formed by them is also less than $\delta$. Specifically, we perform as follows. %Let $n^1_i$ be a node at level 1 and $Siblings(n^1_i)$ be set of siblings of $n^1_i$. For $n^1_j \in Siblings(n^1_i)$, we compare $\textit{rel-supp}(n^1_i, n^1_j)$ with the minimum support threshold (line 9).
Let $n^1_i \in N(1)$. We consider $n^1_i$ with all nodes at level 1 to mine the correlated 2-event patterns. For each $n^1_j \in N(1)$, we compare $\textit{rel-supp}(n^1_i, n^1_j)$ with $\sigma$ (line 9). If $\textit{rel-supp}(n^1_i, n^1_j)$ does not satisfy $\sigma$ then we do not need to find any \textit{pattern nodes} among them. On the contrary, we continue to apply the \textit{property 4.3} of the all-confidence. The node $n^1_j$ is skipped over  if $\frac{supp(n^1_i)}{supp(n^1_j)}$ or $\frac{supp(n^1_j)}{supp(n^1_i)}$ is less than $\delta$ (line 10). Otherwise, we find out all of 2-event patterns between $n^1_i$ and $n^1_j$ (line 11). If there is at least one 2-event pattern such that their relative support and all-confidence are not less than $\sigma$ and $\delta$ respectively, we create a new node $n^2_m$, and keep the bitmap and the maximum support value between $n^1_i$ and $n^1_j$ for optimization in the next levels. Besides, we also insert these 2-event patterns as well as TIIDs respectively into the node $n^2_m$ (lines 12-16).

Moving on to the next levels, the nodes at level (k-1) and level 1 are used to generate the nodes at level k in the patterns enumeration tree. To accelerate the process of mining the correlated k-event patterns, the only nodes at level 1 which exist at level (k-1) do employ to generate the nodes at level k (line 18). This is explained as follows. A node at level k exists, which at least it must satisfy $\sigma$. And both of the node at level 1 and the node at level (k-1) are sub-nodes of the node at level k; therefore, if the node at level 1 does not exist at level (k-1), meaning that it does not satisfy $\sigma$, it leads to the node at level k is also less than $\sigma$. %since it is formed by the node at level 1 and the node at level (k-1).
Consequently, the aforementioned optimization techniques at level 2 are also applied here. Given a node $n^{k-1}_i$ and a node $n^1_j$. We check whether the relative support of $n^{k-1}_i$ and $n^1_j$ is at least $\sigma$ (line 21). If so, we further apply the \textit{property 4.3} of the all-confidence (line 22). 
%If so, we further apply the \textit{property 4.3} of the all-confidence to the generation of k-event patterns. If the ratio of $supp(n^{k-1}_i,n^1_j)$ or $supp(n^1_j)$ to the maximum support value between $n^{k-1}_i$ and $n^1_j$ is less than $\delta$, we do not need to search for k-event patterns (line 23). 
%If this property is satisfied, we seek out all of k-event patterns between $n^{k-1}_i$ and $n^1_j$ (line 24). 
If this property is satisfied, we seek out all of k-event patterns between $n^{k-1}_i$ and $n^1_j$ (line 24). We now explain the way of looking for k-event patterns in function \textit{FindPatterns} (line 31). To mine k-event patterns, we find out the relations between the single events in $n^{k-1}_i$ and $n^1_j$. In this step, we use two properties for optimization: the \textit{transitive property} of the temporal relations and the \textit{property 4.4} of the all-confidence. Assuming that $n^{k-1}_i$ contains $\Sigma_i = \{a_1, a_2, ..., a_{k-1}\}$ and $n^1_j$ contains $\Sigma_j = \{b_1\}$. First, we find out the relations between $a_{k-1}$ and $b_1$ by accessing to the node at level 2 containing $\Sigma=\{a_{k-1}, b_1\}$ and getting 2-event patterns (line 34). If there is no any relations among them, we stop inspecting the temporal relations between $n^{k-1}_i$ and $n^1_j$ (line 39-40). Otherwise, by the \textit{transitive property}, there is a relation between each element in $\{a_1, a_2, ..., a_{k-2}\}$ and $b_1$, and we continue mining process. 
%Throughout this process, if we do not find out a relation which is formed by $a_i \in \Sigma_i$ and $b_1$ such that the ratio of its the support value to the maximum support value between $n^{k-1}_i$ and $n^1_j$ is greater than the minimum all-confidence value, then the k-event pattern between $n^{k-1}_i$ and $n^1_j$ will be not established (lines 36-40). 
Throughout this process, if we do not find out a relation formed by $a_i \in \Sigma_i$ and $b_1$ that satisfies \textit{property 4.4}, then k-event patterns between $n^{k-1}_i$ and $n^1_j$ will be not established (lines 36-40). Applying \textit{transitive property} helps find relations among events quickly since looking for linearly relations among events does not ensure that it exists a relation between each element in $\{a_1, a_2, ..., a_{k-1}\}$ and $b_1$.
Finally, if there is at least one k-event pattern satisfying $\sigma$ and $\delta$, then a new node $n^k_m$ is created and its bitmap and maximum support value are inserted. Moreover, all of k-event patterns along with their TIIDs are also added to node $n^k_m$ (lines 25-29). The algorithm is stopped if we do not find out any the correlated k-event patterns.

%{\SetAlgoNoLine
%\SetNlSty{textbf}{}{:} %set number line in term of 1: , 2: and bold number
\SetNlSty{}{}{:} %set number line in term of 1: , 2:
\begin{algorithm}	
	\algsetup{linenosize=\tiny}
	\SetInd{0.5em}{0.5em}
	\small
	\DontPrintSemicolon
	\caption{The Temporal Patterns Mining OpCTPM}
	\label{algorithmOpTPM}
	
	\KwInput{A set of time series $\mathcal{D}_T$, minimum support threshold $\sigma$, minimum all-confidence threshold $\delta$}
	\KwOutput{The set of the correlated temporal patterns N(k)}
	
	convert $\mathcal{D}_T$ to $D_{Symbol}$ and $D_S$;\;
	\ForEach{\textit{transaction t} $\in \mathcal{D_S}$}{
		\ForEach{\textit{event e} $\in t$}{
			count e's support;\;
			$C1 \gets C1 \cup e$;
		}
	}
	$N(1) \gets \{e \in C1 | \textit{rel-supp}(e) \geq \sigma\}$;\;
	\ForEach{\textit{node} $n^1_i \in N(1)$}{
		%\ForEach{\textit{node} $n^1_j \in Siblings(n^1_i$)}{
		\ForEach{\textit{node} $n^1_j \in N(1)$)}{
			\If{$\textit{rel-supp}(n^1_i,n^1_j) \geq \sigma$}{
				\If{$\frac{supp(n^1_i)}{supp(n^1_j)} \geq \delta$ \textbf{and} $\frac{supp(n^1_j)}{supp(n^1_i)} \geq \delta $}{
					$\small \textit{patterns} \gets \small \text{Find2EventPattern}(n^1_i.\Sigma[0], n^1_j.\Sigma[0])$;\;
					\ForEach{\textit{pattern p} $\in$ \textit{patterns}}{
						\If{$\textit{rel-supp}(p) \geq \sigma$ \textbf{and} \textit{all-conf($p$)} $\geq \delta$}{
							$P^2(n^2_m) \gets P^2(n^2_m) \cup p$;\;
						}
					}
					$n^2_m \gets n^2_m \cup P^2(n^2_m)$;\;
					$N(2) \gets N(2) \cup n^2_m$;\;
				}
			}
		}
	}
	\BlankLine
	\While(\tcp*[h]{$k>2$}) {$N(k-1) \neq \emptyset$} {
		$N^{'}(1) \leftarrow \{n \in N(1) | n$ \textit{exists in} $N(k-1)\} $;\;
		\ForEach{\textit{node} $n^{k-1}_i \in N(k-1)$}{
			\ForEach{\textit{node} $n^1_j \in N^{'}(1)$}{
				\If{$\textit{rel-supp}(n^{k-1}_i,n^1_j) \geq \sigma$}{
					\If{$ \frac{supp(n^{k-1}_i)}{supp(n^1_j)} \geq \delta$ \textbf{and} $\frac{supp(n^1_j)}{supp(n^{k-1}_i)} \geq \delta$}{
						$max \gets max(supp(n^{k-1}_i),supp(n^1_j))$;\;
						$ patterns \gets \text{FindPatterns}(n^{k-1}_i, n^1_j, max)$;\;
						\ForEach{\textit{pattern} $p \in patterns$ }{
							\If{$\textit{rel-supp}(p) \geq \sigma$ \textbf{and} \textit{all-conf($p$)} $\geq \delta$}{
								$P^k(n^k_m) \gets P^k(n^k_m) \cup p$;\;
							}
						}			
						$n^k_m \gets n^k_m \cup P^k(n^k_m)$;\;
						$N(k) \gets N(k) \cup n^k_m$;
					}
				}
			}   		
		}
		$k = k + 1$;
	}
	\BlankLine
	\SetKwFunction{FMain}{FindPaterns}
	\SetKwProg{Fn}{Function}{}{}
	\Fn{\FMain{\textit{Node} $n^{k-1}_i$, \textit{Node} $n^1_j$, $max$}}{
		$P^k(n^k_i) \leftarrow P^{k-1}(n^{k-1}_i)$;\;    
		\For{$x \leftarrow k-1$ \KwTo $1$}{
			$ patterns \leftarrow \text{FindPatterns-Level2}(n^{k-1}_i.\Sigma[x], n^1_j.\Sigma[0])$;\;
			\textit{satisfied-patterns} $\leftarrow \emptyset$;\;
			\ForEach{\textit{pattern} $p \in patterns$}{
				%\If{$\textit{rel-supp}(p) \geq \sigma$}{
				%\If{$\frac{supp(p)}{max\{supp(n^{k-1}_i),supp(n^1_j)\}}\geq \delta$}{
				\If{$\frac{supp(p)}{max}\geq \delta$}{
					\textit{satisfied-patterns} $\leftarrow$ \textit{satisfied-patterns} $\cup  p$;
				}
				%}
			}
			\If{\textit{satisfied-patterns} $= \emptyset$}{
				\textbf{return} $\emptyset$; 
			}
			\Else{
				combine each pattern in \textit{satisfied-patterns} to each pattern in $P^k(n^k_i)$;
			}
		}
		\textbf{return} $P^k(n^k_i)$; 
	}
\end{algorithm}

\hspace{-0.15in}\textbf{Example 5.} Now we clarify the algorithm \ref{algorithmOpTPM} through the following example: consider database $\mathcal{D}_S$ in table \ref{tbl:SequenceDatabase}, given $\sigma=0.7$, $\delta = 0.7$. The patterns enumeration tree in Fig. \ref{fig:patternTree} is the result of this example. We scan $\mathcal{D}_S$ one time and filter the events by $\sigma$, we get $N(1)$=\{A[ON], A[OFF], B[ON], B[OFF], C[ON], C[OFF], D[OFF]\}. At level 2, each node at level 1 is considered with all nodes at level 1 for finding the correlated 2-event patterns. For instance, node A[ON] and node B[ON] are inspected. Since \textit{rel-supp}(A[ON],B[ON]) = 0.75 $\geq \sigma$, \textit{supp}(A[ON]) / \textit{supp}(B[ON]) = 1.33 $\geq \delta$ and \textit{supp}(B[ON]) / \textit{supp}(A[ON]) = 0.75 $\geq \delta$; so we continue looking for the relations between A[ON] and B[ON]. There is a relation among them ``A[ON]$\succcurlyeq$B[ON]" which occurs at temporal sequence ids \{1, 3, 4\}, and \textit{rel-supp}(A[ON]$\succcurlyeq$B[ON]) = 0.75 $\geq \sigma$, \textit{all-conf}(A[ON]$\succcurlyeq$B[ON]) = 0.75 $\geq \delta$; therefore, node \{A[ON], B[ON]\} is created and the pattern node ``A[ON]$\succcurlyeq$B[ON]" as well as its TIID are inserted into node \{A[ON], B[ON]\}. At level 3, each node at level 2 combines with all of nodes at level 1 which exist at level 2. Considering node \{A[ON], B[ON]\} and node \{C[ON]\}, we have $max=max$\{\textit{supp}(A[ON]),\textit{supp}(B[ON]),\textit{supp}(C[ON])\} = 4. Since \textit{rel-supp}(A[ON],B[ON],C[ON]) = 0.75 $\geq \sigma$, \textit{supp}(A[ON],B[ON]) / $max$ = 0.75 $\geq \delta$ and \textit{supp}(C[ON]) / $max$ = 0.75 $\geq \delta$, so we move on searching for the relations between A[ON], B[ON] and C[ON]. As the transitive property of the temporal relations, we first consider the relations between B[ON] and C[ON]. There is a relation B[ON]$\rightarrow$C[ON] and \textit{supp}(B[ON]$\rightarrow$C[ON]) / $max$ =0.75 $\geq \delta$, so there is a relation ``A[ON]$\succcurlyeq$B[ON], B[ON]$\rightarrow$C[ON]". Consequently, we take into account the relations between A[ON] and C[ON]. There is a relation A[ON] $\rightarrow$ C[ON] among them and \textit{supp}(A[ON]$\rightarrow$C[ON]) / $max$ = 0.75 $\geq \delta$. Thus, the node \{A[ON], B[ON]\} and the node \{C[ON]\} form one 3-event pattern ``A[ON]$\succcurlyeq$B[ON], B[ON]$\rightarrow$C[ON], A[ON] $\rightarrow$ C[ON]". The algorithm is stopped until not seeking out any k-event patterns.

\textbf{Time Complexity Analysis.} There are three steps in CTPM composing mining frequent single events, correlated 2-event patterns and correlated k-event patterns $(\text{k}>2$), so we analyse the time complexity for each step. First, to generate the frequent single events, we traverse $\mathcal{D}_S$, and update the support of each event in each temporal sequence of $\mathcal{D}_S$. Assuming that $w$ is the average temporal sequence width, the cost of the operation to find the frequent 1-event patterns requires $O(|\mathcal{D_S}| \cdot w)$. Consequently, to find the correlated 2-event patterns, each event in $N(1)$ is connected with all of events in $N(1)$; and the cost is $O(|N(1)^2|)$. Finally, to achieve the correlated k-event patterns $(\text{k}>2)$, each (k-1)-event patterns at $N(k-1)$ joins each 1-event pattern belonging $N^{'}(1)_{k-1}$, where  $N^{'}(1)_{k-1}$ is the single events belongs $N(1)$ and exists in $N(k-1)$. The cost of finding k-event patterns is $O(\sum_{k=3} |N(k-1)| \cdot |N^{'}(1)_{k-1}|)$. One process which is extremely important in OpCTPM is to find out the temporal relations among the temporal events beginning from level 2 in the patterns enumeration tree. This is based on k-event patterns' TIIDs. Assuming that $m$ is the TIID's average temporal sequence width and $t$ is the TIID's average size. The cost of searching for the relations among $k$ nodes is $t \cdot m^k$. Thus, the complexity of the OpCTPM is ${O\left(\scriptstyle{ |\mathcal{D_S}| \cdot w + |N(1)^2| \cdot t \cdot m^2) + \sum_{k=3} |N(k-1)| \cdot |N^{'}(1)_{k-1}| \cdot t \cdot m^k} \right)}$. However, in practice, due to applying the transitive property of the temporal relations the cost of our algorithm is much lower.

==> boundlambdamu.tex <==
%The following is to put in lemmas. 
We can derive an upper bound for $\lambda_1=p(X_k)$.
\begin{align}
\small
&p(X_i) \geq p(X_k), \forall i \nonumber \\
\Rightarrow &\sum_{i} p(X_i) \geq \sum_{i} p(X_k), \forall i \nonumber\\
\Rightarrow &1 \geq n_x \cdot p(X_k) \nonumber\\
\Rightarrow &p(X_k) \leq \frac{1}{n_x} \nonumber
\end{align}
Hence, $\lambda_1 \leq \frac{1}{n_x}$.

We can derive a upper bound for $\lambda_2=p(X_m,Y_n)$.
\begin{align}
\small
&p(X_i | Y_j) \geq p(X_m | Y_n), \forall i \neq 1 \text{ and } j \neq 1 \nonumber \\
\Rightarrow &p(X_i | Y_j) \cdot p(Y_j) \geq p(X_m | Y_n) \cdot p(Y_j), \forall i \neq 1 \text{ and } j \neq 1 \nonumber
\end{align}
\begin{align}
\small
\Rightarrow \sum_{i\neq1} \sum_{j\neq1} p(X_i | Y_j) \cdot p(Y_j) &\geq \sum_{i\neq1} \sum_{j\neq1} p(X_m | Y_n) \cdot p(Y_j) \nonumber \\ 
&=p(X_m | Y_n) \cdot \sum_{i\neq1} \sum_{j\neq1}  p(Y_j) \nonumber \\ 
&=p(X_m | Y_n) \cdot (n_x -p(Y_1)) \nonumber \\
&\geq p(X_m | Y_n) \cdot (n_x -1) \nonumber
\end{align}
\begin{align}
\small
\Rightarrow p(X_m | Y_n) & \leq \frac{\sum_{i\neq1} \sum_{j\neq1} p(X_i | Y_j) \cdot p(Y_j) }{n_x - 1} \nonumber \\
&= \frac{\sum_{i\neq1} \sum_{j\neq1} p(X_i , Y_j)} {n_x - 1} \nonumber \\
&= \frac{1-p(X_1,Y_1)}{n_x - 1} \nonumber \\ 
&\leq \frac{1-\sigma}{n_x - 1} \nonumber 
\end{align}
$\Rightarrow p(X_m,Y_n) \leq p(Y_n) \cdot \frac{1-\sigma}{n_x - 1}  \leq \frac{(1-\sigma)}{n_x - 1}  \nonumber$

Hence, $\lambda_2 \leq \frac{(1-\sigma)}{n_x - 1}$.

We can derive a lower bound of $\mu$.

\begin{align}
\small
\textit{conf}(X_1,Y_1)_{\mathcal{D}_{\text{SEQ}}} \geq \lambda_1^{\frac{1-\mu}{\sigma}} \cdot \left(\frac{n_x - 1}{1-\sigma}\right)^{\frac{\lambda_2}{\sigma}} \cdot \sigma \geq \gamma \nonumber
\end{align}
\begin{align}
\small
\Leftrightarrow \lambda_1^{\frac{1-\mu}{\sigma}} &\geq \frac{\gamma}{\sigma} \cdot \left(\frac{1-\sigma}{n_x - 1}\right)^{\frac{\lambda_2}{\sigma}} \nonumber \\
\Leftrightarrow \lambda_1^{\frac{1-\mu}{\sigma}} &\geq \lambda_1^{\log_{\lambda_1}{\left(\frac{\gamma}{\sigma} \cdot \left(\frac{1-\sigma}{n_x - 1}\right)^{\frac{\lambda_2}{\sigma}}\right)}} \nonumber \\
\Leftrightarrow \frac{1-\mu}{\sigma} &\leq \log_{\lambda_1}{\left(\frac{\gamma}{\sigma} \cdot \left(\frac{1-\sigma}{n_x - 1}\right)^{\frac{\lambda_2}{\sigma}}\right)} (0<\lambda_1<1) \nonumber \\ 
\Leftrightarrow \mu &\geq 1-\sigma \cdot  \log_{\lambda_1}{\left(\frac{\gamma}{\sigma} \cdot \left(\frac{1-\sigma}{n_x - 1}\right)^{\frac{\lambda_2}{\sigma}}\right)}
\end{align}

==> combine/code_noscale.tex <==
\begin{figure*}
	\setlength{\tabcolsep}{0pt}
	\begin{tabularx}{\linewidth}{ll}
		\begin{minipage}{.3\linewidth}
			\begin{minipage}{\linewidth}
				\resizebox{\linewidth}{.8\linewidth}{%
					\input{combine/framework.tex}
				}
				\caption{Overview of FTPMfTS process}
				\label{fig:framework}
			\end{minipage}
			\\
			\phantom{unvisibility}
			\\
			\\
			\begin{subfigure}[b]{\linewidth}
				%\begin{minipage}{\linewidth}
				\resizebox{\linewidth}{.95cm}{%
					\input{combine/noneOverlap.tex}
				}
				\caption{With no overlapping}
				\label{fig:basicSplit}
				%\end{minipage}
			\end{subfigure}
			\\
			\begin{subfigure}[b]{\linewidth}
				%\begin{minipage}{\linewidth}
				\resizebox{\linewidth}{1.3cm}{%
					\input{combine/overlap.tex}
				}
				\caption{With overlapping}
				\label{fig:overlaptransaction2}
				%\end{minipage}
			\end{subfigure}
			\caption{Splitting strategy}
			\label{fig:splitting}
		\end{minipage}&
		\hspace{0.5in}
		\begin{minipage}{.6\linewidth}
		%	\phantom{unvisibility}
		%	\\
		%	\phantom{unvisibility}
		%	\\
		%	\phantom{unvisibility}
		%	\\
		%	\phantom{unvisibility}
		%	\\
			\resizebox{\linewidth}{8.2cm}{%
				\includegraphics[width=\textwidth]{combine/enumerationTree.pdf}
			}
				\caption{A Hierarchical Pattern Graph for Table  \ref{tbl:SequenceDatabase}}
				\label{fig:patternTree}
		\end{minipage}
	\end{tabularx}
\end{figure*}


==> data/combineFigure/code.tex <==
\begin{figure*}
	\setlength{\tabcolsep}{0pt}
	\begin{tabularx}{\linewidth}{ll}
		\begin{minipage}{.35\linewidth}
			\begin{minipage}{\linewidth}
				\resizebox{\linewidth}{\linewidth}{%
					\input{data/combineFigure/framework.tex}
				}
				\caption{Overview of FTPMfTS process}
				\label{fig:framework}
			\end{minipage}
			\\
			
			\begin{subfigure}[b]{\linewidth}
				%\begin{minipage}{\linewidth}
				\resizebox{\linewidth}{.98cm}{%
					\input{data/combineFigure/noneOverlap.tex}
				}
				\caption{With no overlapping}
				\label{fig:basicSplit}
				%\end{minipage}
			\end{subfigure}
			\\
			\begin{subfigure}[b]{\linewidth}
				%\begin{minipage}{\linewidth}
				\resizebox{\linewidth}{1.3cm}{%
					\input{data/combineFigure/overlap.tex}
				}
				\caption{With overlapping}
				\label{fig:overlaptransaction2}
				%\end{minipage}
			\end{subfigure}
			\caption{Splitting strategy}
			\label{fig:splitting}
		\end{minipage}&
		\begin{minipage}{.65\linewidth}
			\resizebox{\linewidth}{8.5cm}{%
				\includegraphics[width=\textwidth]{data/combineFigure/enumerationTree.pdf}
			}
				\caption{A Hierarchical Pattern Graph for Table  \ref{tbl:SequenceDatabase}}
				\label{fig:patternTree}
		\end{minipage}
	\end{tabularx}
\end{figure*}


==> data/combineFigure/framework.tex <==

\tikzstyle{arrow} = [black,opacity=1,thin,-{Triangle[angle=60:1.2mm]}]
\tikzstyle{line} = [black,opacity=1,thin,dotted]
\tikzstyle{box} = [rectangle,rounded corners, minimum width=7cm, minimum height=0.5cm, text centered,text width = 7cm, draw=black, text opacity=1]
\tikzstyle{bounding1} = [rectangle, dotted, minimum width=8.5cm, minimum height=2.4cm, draw=black, fill=blue, text opacity=1]
\tikzstyle{bounding2} = [rectangle,dotted, minimum width=8.5cm, minimum height=3.2cm, draw=black, fill=green, text opacity=1]
\tikzstyle{textlabel} = [text centered,text width = 3cm, text opacity=1, rotate=270, yshift = -12]
\begin{tikzpicture}[node distance=-1.5cm, fill opacity=0.2]
\tikzstyle{arrow} = [black,opacity=1,thin,-{Triangle[angle=60:1.2mm]}]
\tikzstyle{line} = [black,opacity=1,thin,dotted]
\tikzstyle{box} = [rectangle,rounded corners, minimum width=5.6cm, minimum height=0.5cm, text centered,text width = 5.6cm, draw=black, text opacity=1]
\tikzstyle{bounding1} = [rectangle, dotted, minimum width=7cm, minimum height=2.4cm, draw=black, fill=blue, text opacity=1]
\tikzstyle{bounding2} = [rectangle,dotted, minimum width=7cm, minimum height=3.2cm, draw=black, fill=green, text opacity=1]
\tikzstyle{bounding3} = [rectangle,dotted, minimum width=8cm, minimum height=6cm, draw=black, fill=teal, text opacity=1]
\tikzstyle{textlabel} = [text centered,text width = 3cm, text opacity=1, rotate=270, yshift = -12]
\tikzstyle{textlabel2} = [text centered,text width = 3cm, text opacity=1, rotate=90, yshift = -10]
\node (A) [box, fill=red] {\small Set of Time Series $\mathcal{X}$};
%		\node [boundingA, left of=boundA] {\small {Data Transformation}} ;
%

\node (B) [box, below of=A, yshift=-2.6cm] {\small Symbolic Time Series Representation};
\node (C) [box, below of=B, yshift=-2.6cm] {\small Temporal Sequence Database Conversion};
%		\node (boundB) [bounding2, above of=A, yshift=-2.8cm] {};
\node (D) [box, below of=C, yshift=-2.9cm] {\small Frequent Single Event Mining};
\node (E) [box, below of=D, yshift=-2.5cm] {\small Frequent 2-Event Pattern Mining};
\node (F) [box, below of=E, yshift=-2.5cm] {\small Frequent k-Event Pattern Mining (k $>2$)};

\node (boundingC) [bounding3, fit=(B) (C) (D) (E) (F),  xshift=0cm] {};
\draw [line] ($(boundingC.north) + (3.2cm,0)$) -- node [black, textlabel2] {\small FTPMfTS Process}  ($(boundingC.south) + (3.2cm,0)$);

\node (boundingA)[bounding1, fit=(B) (C), xshift=-.4cm] {};
\draw [line] ($(boundingA.north) - (2.6cm,0)$) -- node [black, textlabel] {\small \phantom{abc}Data\phantom{abc} Transformation }  ($(boundingA.south) - (2.6cm,0)$);

\node (boundingB)[bounding2, fit=(D) (E) (F), xshift=-.4cm] {};
\draw [line] ($(boundingB.north) - (2.6cm,0)$) -- node [black, textlabel] {\small Temporal Patterns Mining (HTPGM)}  ($(boundingB.south) - (2.6cm,0)$);

\node (G) [box, fill=red, below of=F, yshift=-2.7cm] {\small Frequent Temporal Patterns};
\draw[arrow] (A) -- (B) ;
\draw[arrow] (B) -- node[anchor=west] {$\mathcal{D}_{\text{SYB}}$} (C) ;
\draw[arrow] (C) -- node[anchor=west] {$\mathcal{D}_{\text{SEQ}}$} (D) ;
\draw[arrow] (D) -- (E) ;
\draw[arrow] (E) -- (F) ;
\draw[arrow] (F) -- (G) ;
\end{tikzpicture}








==> data/combineFigure/noneOverlap.tex <==
\definecolor{arrowcolor}{rgb}{.27,.45,.77}
\tikzstyle{arrow} = [arrowcolor,opacity=1,thin, {Triangle[angle=60:1.2mm]}-{Triangle[angle=60:1.2mm]}]
\tikzstyle{roundrect} = [rectangle,rounded corners, minimum width=6cm, minimum height=0.8cm, text centered,text width =1.4cm, draw=white, fill=white, text opacity=1]
\tikzstyle{roundrect3} = [rectangle,rounded corners, minimum width=3cm, minimum height=0.8cm, text centered,text width =1.4cm, draw=black, fill=red, text opacity=1, fill opacity=.15]
\tikzstyle{roundrect4} = [rectangle,rounded corners, minimum width=3cm, minimum height=0.8cm, text centered,text width =1.4cm, draw=black, fill=blue, text opacity=1, fill opacity=.3]
\tikzstyle{line} = [black,opacity=1,thin, {Circle[scale=0.4]}-{Circle[scale=0.4]}]

\begin{tikzpicture}[fill opacity=.2]
\node (bbox) [roundrect] {};
\node (anode) [roundrect3, left of=bbox, xshift=-.5cm] {};
\node (cnode) [roundrect4,  left of=anode, xshift = 4cm] {};
\node [text opacity=1] at ($(anode.west)!0.5!(cnode.west)$) {$S_1$} ;
\node [text opacity=1] at ($(anode.east)!0.5!(cnode.east)$) {$S_2$} ;
%\draw [arrow] ($(cnode.west)+(0,1.2)$) -- node [black, below,yshift=2] {\small t\textsubscript{max}}  ($(anode.east)+(0,1.2)$);
\draw [arrow] ($(anode.west)+(0,.6)$) -- node [black, above, yshift=-2] {\small $t$}   ($(anode.east)+(0,.6)$);
\draw [arrow] ($(cnode.west)+(0,.6)$) -- node [black, above, yshift=-2] {\small $t$}   ($(cnode.east)+(0,.6)$);

\draw [line] ($(anode.east)+(-.01,.2)$) -- node [black, above,yshift=-2.5] {\tiny KOn}  ($(anode.east)+(-1,.2)$);
\draw [line] ($(anode.east)+(-.01,.0)$) -- node [black, above,yshift=-2.5] {\tiny TOn}  ($(anode.east)+(-1,.0)$);
\draw [line] ($(cnode.west)+(.01,-.1)$) -- node [black, above,yshift=-2.5] {\tiny MOn}  ($(cnode.west)+(.8,-.1)$);
\draw [line] ($(cnode.west)+(.01,-.3)$) -- node [black, above,yshift=-2.5] {\tiny COn}  ($(cnode.west)+(.8,-.3)$);
\end{tikzpicture}

==> data/combineFigure/overlap.tex <==
\definecolor{arrowcolor}{rgb}{.27,.45,.77}
\tikzstyle{arrow} = [arrowcolor,opacity=1,thin, {Triangle[angle=60:1.2mm]}-{Triangle[angle=60:1.2mm]}]
\tikzstyle{roundrect} = [rectangle,rounded corners, minimum width=6cm, minimum height=.8cm, text centered,text width =1.4cm, draw=white, fill=white, text opacity=1]
\tikzstyle{roundrect3} = [rectangle, rounded corners, minimum width=3cm, minimum height=.8cm, text centered,text width =1.4cm, draw=black, fill=red, text opacity=1, dashed, fill opacity=.15]
\tikzstyle{roundrect4} = [rectangle,rounded corners, minimum width=3cm, minimum height=.8cm, text centered,text width =1.4cm, draw=black, fill=blue, text opacity=1, fill opacity=.3]
\tikzstyle{line} = [black,opacity=1,thin, {Circle[scale=0.4]}-{Circle[scale=0.4]}]

\begin{tikzpicture}[fill opacity=.2]
\node (bbox) [roundrect] {};
\node (anode) [roundrect3, left of=bbox, xshift=-.5cm] {};
%\draw [rounded corners] (0,0) -- (4,0) -- (4,4) -- (0,4);
\draw [rounded corners] ($(anode.south east) + (-0.5,.007)$) --  ($(anode.south west) + (.007,.007)$) -- ($(anode.north west) + (.007,-.007)$)--  ($(anode.north east) - (-0.5,.007)$);

\node (cnode) [roundrect4,  left of=anode, xshift = 3cm] {};
\node [text opacity=1] at ($(anode.west)!0.6!(cnode.west)$) {$S_1$} ;
\node [text opacity=1] at ($(anode.east)!0.7!(cnode.east)$) {$S_2$} ;
\draw [arrow] ($(cnode.west)+(0,.48)$) -- node [black, above,yshift=-2] {\small $t_{o}$}  ($(anode.east)+(0,.48)$);
\draw [arrow] ($(anode.west)+(0,.8)$) -- node [black, above, yshift=-2] {\small $t$}   ($(anode.east)+(0,.8)$);
\draw [arrow] ($(cnode.west)+(0,1)$) -- node [black, above, yshift=-2] {\small $t$}   ($(cnode.east)+(0,1)$);


\draw [line] ($(cnode.west)+(.01,.2)$) -- node [black, above,yshift=-2.5] {\tiny KOn}  ($(cnode.west)+(1,.2)$);
\draw [line] ($(cnode.west)+(.01,0)$) -- node [black, above,yshift=-2.5] {\tiny TOn}  ($(cnode.west)+(1,0)$);
\draw [line] ($(anode.east)+(.01,-.1)$) -- node [black, above,yshift=-2.5] {\tiny MOn}  ($(anode.east)+(.8,-.1)$);
\draw [line] ($(anode.east)+(.01,-.3)$) -- node [black, above,yshift=-2.5] {\tiny COn}  ($(anode.east)+(.8,-.3)$);
\end{tikzpicture}

==> data/framework.tex <==

\tikzstyle{arrow} = [black,opacity=1,thin,-{Triangle[angle=60:1.2mm]}]
\tikzstyle{line} = [black,opacity=1,thin,dotted]
\tikzstyle{box} = [rectangle,rounded corners, minimum width=7cm, minimum height=0.5cm, text centered,text width = 7cm, draw=black, text opacity=1]
\tikzstyle{bounding1} = [rectangle, dotted, minimum width=8.5cm, minimum height=2.4cm, draw=black, fill=blue, text opacity=1]
\tikzstyle{bounding2} = [rectangle,dotted, minimum width=8.5cm, minimum height=3.2cm, draw=black, fill=green, text opacity=1]
\tikzstyle{textlabel} = [text centered,text width = 3cm, text opacity=1, rotate=270, yshift = -12]
\begin{tikzpicture}[node distance=-1.5cm, fill opacity=0.2]
\tikzstyle{arrow} = [black,opacity=1,thin,-{Triangle[angle=60:1.2mm]}]
\tikzstyle{line} = [black,opacity=1,thin,dotted]
\tikzstyle{box} = [rectangle,rounded corners, minimum width=5.6cm, minimum height=0.5cm, text centered,text width = 5.6cm, draw=black, text opacity=1]
\tikzstyle{bounding1} = [rectangle, dotted, minimum width=7cm, minimum height=2.4cm, draw=black, fill=blue, text opacity=1]
\tikzstyle{bounding2} = [rectangle,dotted, minimum width=7cm, minimum height=3.2cm, draw=black, fill=green, text opacity=1]
\tikzstyle{bounding3} = [rectangle,dotted, minimum width=8cm, minimum height=6cm, draw=black, fill=teal, text opacity=1]
\tikzstyle{textlabel} = [text centered,text width = 3cm, text opacity=1, rotate=270, yshift = -12]
\tikzstyle{textlabel2} = [text centered,text width = 3cm, text opacity=1, rotate=90, yshift = -10]
\node (A) [box, fill=red] {\small Set of Time Series $\mathcal{X}$};
%		\node [boundingA, left of=boundA] {\small {Data Transformation}} ;
%

\node (B) [box, below of=A, yshift=-2.6cm] {\small Symbolic Time Series Representation};
\node (C) [box, below of=B, yshift=-2.6cm] {\small Temporal Sequence Database Conversion};
%		\node (boundB) [bounding2, above of=A, yshift=-2.8cm] {};
\node (D) [box, below of=C, yshift=-2.9cm] {\small Frequent Single Event Mining};
\node (E) [box, below of=D, yshift=-2.5cm] {\small Frequent 2-Event Pattern Mining};
\node (F) [box, below of=E, yshift=-2.5cm] {\small Frequent k-Event Pattern Mining (k $>2$)};

\node (boundingC) [bounding3, fit=(B) (C) (D) (E) (F),  xshift=0cm] {};
\draw [line] ($(boundingC.north) + (3.2cm,0)$) -- node [black, textlabel2] {\small FTPMfTS Process}  ($(boundingC.south) + (3.2cm,0)$);

\node (boundingA)[bounding1, fit=(B) (C), xshift=-.4cm] {};
\draw [line] ($(boundingA.north) - (2.6cm,0)$) -- node [black, textlabel] {\small \phantom{abc}Data\phantom{abc} Transformation }  ($(boundingA.south) - (2.6cm,0)$);

\node (boundingB)[bounding2, fit=(D) (E) (F), xshift=-.4cm] {};
\draw [line] ($(boundingB.north) - (2.6cm,0)$) -- node [black, textlabel] {\small Temporal Patterns Mining (HTPGM)}  ($(boundingB.south) - (2.6cm,0)$);

\node (G) [box, fill=red, below of=F, yshift=-2.7cm] {\small Frequent Temporal Patterns};
\draw[arrow] (A) -- (B) ;
\draw[arrow] (B) -- node[anchor=west] {$\mathcal{D}_{\text{SYB}}$} (C) ;
\draw[arrow] (C) -- node[anchor=west] {$\mathcal{D}_{\text{SEQ}}$} (D) ;
\draw[arrow] (D) -- (E) ;
\draw[arrow] (E) -- (F) ;
\draw[arrow] (F) -- (G) ;
\end{tikzpicture}








==> data/overlapping/noneOverlap.tex <==
\definecolor{arrowcolor}{rgb}{.27,.45,.77}
\tikzstyle{arrow} = [arrowcolor,opacity=1,thin, {Triangle[angle=60:1.2mm]}-{Triangle[angle=60:1.2mm]}]
\tikzstyle{roundrect} = [rectangle,rounded corners, minimum width=6cm, minimum height=1.2cm, text centered,text width =1.4cm, draw=white, fill=white, text opacity=1]
\tikzstyle{roundrect3} = [rectangle,rounded corners, minimum width=3cm, minimum height=1.2cm, text centered,text width =1.4cm, draw=black, fill=red, text opacity=1, fill opacity=.15]
\tikzstyle{roundrect4} = [rectangle,rounded corners, minimum width=3cm, minimum height=1.2cm, text centered,text width =1.4cm, draw=black, fill=blue, text opacity=1, fill opacity=.3]
\tikzstyle{line} = [black,opacity=1,thin, {Circle[scale=0.4]}-{Circle[scale=0.4]}]

\begin{tikzpicture}[fill opacity=.2]
\node (bbox) [roundrect] {};
\node (anode) [roundrect3, left of=bbox, xshift=-.5cm] {};
\node (cnode) [roundrect4,  left of=anode, xshift = 4cm] {};
\node [text opacity=1] at ($(anode.west)!0.5!(cnode.west)$) {$S_1$} ;
\node [text opacity=1] at ($(anode.east)!0.5!(cnode.east)$) {$S_2$} ;
%\draw [arrow] ($(cnode.west)+(0,1.2)$) -- node [black, below,yshift=2] {\small t\textsubscript{max}}  ($(anode.east)+(0,1.2)$);
\draw [arrow] ($(anode.west)+(0,.8)$) -- node [black, above, yshift=-2] {\small $t$}   ($(anode.east)+(0,.8)$);
\draw [arrow] ($(cnode.west)+(0,.8)$) -- node [black, above, yshift=-2] {\small $t$}   ($(cnode.east)+(0,.8)$);

\draw [line] ($(anode.east)+(-.01,.4)$) -- node [black, above,yshift=-2.5] {\tiny KOn}  ($(anode.east)+(-.6,.4)$);
\draw [line] ($(anode.east)+(-.01,.2)$) -- node [black, above,yshift=-2.5] {\tiny TOn}  ($(anode.east)+(-.6,.2)$);
\draw [line] ($(cnode.west)+(.01,0)$) -- node [black, above,yshift=-2.5] {\tiny MOn}  ($(cnode.west)+(.4,0)$);
\draw [line] ($(cnode.west)+(.01,-.2)$) -- node [black, above,yshift=-2.5] {\tiny COn}  ($(cnode.west)+(.4,-.2)$);
\end{tikzpicture}

==> data/overlapping/overlap.tex <==
\definecolor{arrowcolor}{rgb}{.27,.45,.77}
\tikzstyle{arrow} = [arrowcolor,opacity=1,thin, {Triangle[angle=60:1.2mm]}-{Triangle[angle=60:1.2mm]}]
\tikzstyle{roundrect} = [rectangle,rounded corners, minimum width=6cm, minimum height=1.2cm, text centered,text width =1.4cm, draw=white, fill=white, text opacity=1]
\tikzstyle{roundrect3} = [rectangle, rounded corners, minimum width=3cm, minimum height=1.2cm, text centered,text width =1.4cm, draw=black, fill=red, text opacity=1, dashed, fill opacity=.15]
\tikzstyle{roundrect4} = [rectangle,rounded corners, minimum width=3cm, minimum height=1.2cm, text centered,text width =1.4cm, draw=black, fill=blue, text opacity=1, fill opacity=.3]
\tikzstyle{line} = [black,opacity=1,thin, {Circle[scale=0.4]}-{Circle[scale=0.4]}]

\begin{tikzpicture}[fill opacity=.2]
\node (bbox) [roundrect] {};
\node (anode) [roundrect3, left of=bbox, xshift=-.5cm] {};
%\draw [rounded corners] (0,0) -- (4,0) -- (4,4) -- (0,4);
\draw [rounded corners] ($(anode.south east) + (-0.5,.007)$) --  ($(anode.south west) + (.007,.007)$) -- ($(anode.north west) + (.007,-.007)$)--  ($(anode.north east) - (-0.5,.007)$);

\node (cnode) [roundrect4,  left of=anode, xshift = 3.4cm] {};
\node [text opacity=1] at ($(anode.west)!0.6!(cnode.west)$) {$S_1$} ;
\node [text opacity=1] at ($(anode.east)!0.4!(cnode.east)$) {$S_2$} ;
\draw [arrow] ($(cnode.west)+(0,.7)$) -- node [black, above,yshift=-2] {\small $t_{o}$}  ($(anode.east)+(0,.7)$);
\draw [arrow] ($(anode.west)+(0,1)$) -- node [black, above, yshift=-2] {\small $t$}   ($(anode.east)+(0,1)$);
\draw [arrow] ($(cnode.west)+(0,1.2)$) -- node [black, above, yshift=-2] {\small $t$}   ($(cnode.east)+(0,1.2)$);


\draw [line] ($(cnode.west)+(.01,.4)$) -- node [black, above,yshift=-2.5] {\tiny KOn}  ($(cnode.west)+(.6,.4)$);
\draw [line] ($(cnode.west)+(.01,.2)$) -- node [black, above,yshift=-2.5] {\tiny TOn}  ($(cnode.west)+(.6,.2)$);
\draw [line] ($(anode.east)+(.01,0)$) -- node [black, above,yshift=-2.5] {\tiny MOn}  ($(anode.east)+(.4,0)$);
\draw [line] ($(anode.east)+(.01,-.2)$) -- node [black, above,yshift=-2.5] {\tiny COn}  ($(anode.east)+(.4,-.2)$);
\end{tikzpicture}

==> data/overlapping/overlapV1.tex <==
\definecolor{arrowcolor}{rgb}{.27,.45,.77}
\tikzstyle{arrow} = [arrowcolor,opacity=1,thin, {Triangle[angle=60:1.2mm]}-{Triangle[angle=60:1.2mm]}]
\tikzstyle{roundrect} = [rectangle,rounded corners, minimum width=6cm, minimum height=1.2cm, text centered,text width =1.4cm, draw=white, fill=white, text opacity=1]
\tikzstyle{roundrect3} = [rectangle,rounded corners, minimum width=3cm, minimum height=1.2cm, text centered,text width =1.4cm, draw=black, fill=red, text opacity=1]
\tikzstyle{roundrect4} = [rectangle,rounded corners, minimum width=3cm, minimum height=1.2cm, text centered,text width =1.4cm, draw=black, fill=blue, text opacity=1]
\tikzstyle{line} = [black,opacity=1,thin, {Circle[scale=0.4]}-{Circle[scale=0.4]}]

\begin{tikzpicture}[fill opacity=.2]
\node (bbox) [roundrect] {};
\node (anode) [roundrect3, left of=bbox, xshift=-.5cm] {};
\node (cnode) [roundrect4,  left of=anode, xshift = 3.4cm] {};
\node [text opacity=1] at ($(anode.west)!0.6!(cnode.west)$) {$S_1$} ;
\node [text opacity=1] at ($(anode.east)!0.4!(cnode.east)$) {$S_2$} ;
\draw [arrow] ($(cnode.west)+(0,.7)$) -- node [black, above,yshift=-2] {\small $t_{o}$}  ($(anode.east)+(0,.7)$);
\draw [arrow] ($(anode.west)+(0,1)$) -- node [black, above, yshift=-2] {\small $t$}   ($(anode.east)+(0,1)$);

\draw [line] ($(cnode.west)+(.01,.4)$) -- node [black, above,yshift=-2.5] {\tiny KOn}  ($(cnode.west)+(.6,.4)$);
\draw [line] ($(cnode.west)+(.01,.2)$) -- node [black, above,yshift=-2.5] {\tiny TOn}  ($(cnode.west)+(.6,.2)$);
\draw [line] ($(anode.east)+(.01,0)$) -- node [black, above,yshift=-2.5] {\tiny MOn}  ($(anode.east)+(.4,0)$);
\draw [line] ($(anode.east)+(.01,-.2)$) -- node [black, above,yshift=-2.5] {\tiny COn}  ($(anode.east)+(.4,-.2)$);
\end{tikzpicture}

==> data/sax/SAX.tex <==
\begin{tikzpicture}[node distance=-1.5cm]
\tikzstyle{arrow} = [black,opacity=1,-{Triangle[angle=60:1.2mm]}]
\tikzstyle{cell} = [minimum width=.9cm,minimum height=0.85cm, text width=.9cm, text centered, align=center]
\tikzstyle{cell2} = [minimum width=2cm,minimum height=0.85cm, text width=4.3cm, text centered, align=center]
\tikzstyle{cell3} = [minimum width=1cm,minimum height= 2cm]
\definecolor{col1}{rgb}{1, 0.9, 0.6}
\tikzstyle{color1} = [fill=col1]
\definecolor{col2}{rgb}{0.49,0.65,0.88}
\tikzstyle{color2} = [fill=col2]
\definecolor{col3}{rgb}{0.8,1,0.8}
\tikzstyle{color3} = [fill=col3]

% sX,eX,Y
\newcommand{\DrawON}[3]{
%	\draw [black] (axis cs: #1, #3+1) -- (axis cs: #2, #3+1);
    \node [black, scale=0.6] at (axis cs: #1/2+#2/2, #3+2.5) {\large On};
}
% sX,eX,Y
\newcommand{\DrawOFF}[3]{
%	\draw [black] (axis cs: #1, #3+1) -- (axis cs: #2, #3+1);
	\node [black, scale=0.6] at (axis cs: #1/2+#2/2, #3+2.5) {\large Off};
}

\matrix (row1) [matrix of nodes,nodes={cell},column sep=-\pgflinewidth]{
	|[draw]| \footnotesize 0.10 & |[draw]| \footnotesize 0.13 & |[draw]| \footnotesize 0.24 & |[draw]| \footnotesize 0.25 & |[draw]| \footnotesize 1.15 & |[draw]| \footnotesize 1.15 & |[draw]| \footnotesize 1.16 & |[draw]| \footnotesize 1.14 & |[draw]| \footnotesize 0.35 & |[draw]| \footnotesize 0.43 & |[draw]| \footnotesize 0.32 & |[draw]| \footnotesize 0.22 & |[draw]| \footnotesize 0.89 & |[draw]| \footnotesize  0.97 & |[draw]| \footnotesize 1.12 & |[draw]| \footnotesize 1.12 \\
};

\begin{axis}[axis line style={draw=none},
	tick style={draw=none},
	ymin = 0, ymax = 10,
	xmin = 0, xmax = 200,
	xticklabels={,,},
	yticklabels={,,},
	yscale=0.15,
	xscale=2.64,
	at={($(row1.north west)+(.1cm,0.2cm)$)}
]
\addplot [mark=none, color=orange, very thick] table [x=x, y=y, col sep=comma] {data/sax/a.csv};
\DrawOFF{1}{49}{0}
\DrawON{51}{100}{5}
\DrawOFF{102}{149}{0}
\DrawON{151}{200}{5}
\end{axis}

\matrix (row2) [matrix of nodes,nodes={cell},column sep=-\pgflinewidth, above of=row1]{
	|[draw,color3]| \footnotesize Off & |[draw,color3]| \footnotesize Off & |[draw,color3]| \footnotesize Off & |[draw,color3]| \footnotesize Off & |[draw,color1]| \footnotesize On & |[draw,color1]| \footnotesize On & |[draw,color1]| \footnotesize On & |[draw,color1]| \footnotesize On & |[draw,color3]| \footnotesize Off & |[draw,color3]| \footnotesize Off & |[draw,color3]| \footnotesize Off & |[draw,color3]| \footnotesize Off & |[draw,color1]| \footnotesize On & |[draw,color1]| \footnotesize  On & |[draw,color1]| \footnotesize On & |[draw,color1]| \footnotesize On \\
};

\matrix (row3) [matrix of nodes,nodes={cell2},column sep=-\pgflinewidth,row sep=-\pgflinewidth, above of=row2]{
	|[draw,color3]| \footnotesize Off & |[draw,color1]| \footnotesize On  & |[draw,color3]| \footnotesize Off & |[draw,color1]| \footnotesize On \\
};
\node [right of=row1, xshift=-9.3cm] {\small \phantom{ooooio}Time Series\phantom{moooo}};
\node [right of=row2, xshift=-9.3cm] {\small Symbolic Representation};
\node [right of=row3, xshift=-9.3cm] {\small \phantom{oooo}Temporal Event\phantom{oooo}};

\matrix (column) [matrix of nodes,nodes={cell3},column sep=-\pgflinewidth,row sep=-\pgflinewidth, left of=row2, xshift = 9cm]{
	|[draw,color1]| \small On \\
	|[draw,color3]| \small Off \\
};
\node at ($(column-1-1.north west) - (.4,0)$) {+$\infty$};
\node at ($(column-2-1.north west) - (.4,0)$) {$0.5$};
\node at ($(column-2-1.south west) - (.3,0)$) {-$\infty$};

\draw[arrow] (row1-1-1) -- (row2-1-1);
\draw[arrow] (row1-1-2) -- (row2-1-2);
\draw[arrow] (row1-1-3) -- (row2-1-3);
\draw[arrow] (row1-1-4) -- (row2-1-4);
\draw[arrow] (row1-1-5) -- (row2-1-5);
\draw[arrow] (row1-1-6) -- (row2-1-6);
\draw[arrow] (row1-1-7) -- (row2-1-7);
\draw[arrow] (row1-1-8) -- (row2-1-8);
\draw[arrow] (row1-1-9) -- (row2-1-9);
\draw[arrow] (row1-1-10) -- (row2-1-10);
\draw[arrow] (row1-1-11) -- (row2-1-11);
\draw[arrow] (row1-1-12) -- (row2-1-12);
\draw[arrow] (row1-1-13) -- (row2-1-13);
\draw[arrow] (row1-1-14) -- (row2-1-14);
\draw[arrow] (row1-1-15) -- (row2-1-15);
\draw[arrow] (row1-1-16) -- (row2-1-16);
\draw[arrow] ($(row2-1-3.south)!0.5!(row2-1-2.south)$) -- (row3-1-1);
\draw[arrow] ($(row2-1-7.south)!0.5!(row2-1-6.south)$) -- (row3-1-2);
\draw[arrow] ($(row2-1-11.south)!0.5!(row2-1-10.south)$) -- (row3-1-3);
\draw[arrow] ($(row2-1-15.south)!0.5!(row2-1-14.south)$) -- (row3-1-4);


\end{tikzpicture}

==> data/tikz/timeSeries.tex <==
\begin{tikzpicture}


% sX,eX,Y
\newcommand{\DrawON}[3]{
    \draw [black,thin] (axis cs: #1, #3+0.15) -- (axis cs: #2, #3+0.15);
    \node [black, scale=0.6] at (axis cs: #1/2+#2/2, #3+0.35) {\scriptsize On};
}
% sX,eX,Y
\newcommand{\DrawOFF}[3]{
    \draw [black,thin] (axis cs: #1, #3-0.2) -- (axis cs: #2, #3-0.2);
    \node [black, scale=0.6] at (axis cs: #1/2+#2/2, #3-0.45) {\scriptsize Off};
}
% sX,eX,Y, Shift
\newcommand{\DrawOFFSHIFT}[4]{
    \draw [black,thin] (axis cs: #1, #3-0.2) -- (axis cs: #2, #3-0.2);
    \node [black, scale=0.6] at (axis cs: #1/2+#2/2+#4, #3-0.45) {\scriptsize Off};
}


\begin{axis}[axis line style={draw=none},
             tick style={draw=none},
             ymin = -2.5, ymax = 6,
             xmin = -200, xmax = 950,
             xticklabels={,,},
             yticklabels={,,},
             yscale=0.35
             ]

\draw [black, thin, -latex] (axis cs: 0, -1) -- (axis cs: 950,-1) node [right] {};

\addplot [mark=none, color=cyan] table [x=x, y=microwave, col sep=comma] {data/tikz/newdataTimeSeries.csv};
\addplot [mark=none, color=orange] table [x=x, y=toaster, col sep=comma] {data/tikz/newdataTimeSeries.csv};
\addplot [mark=none, color=teal] table [x=x, y=kitchen, col sep=comma] {data/tikz/newdataTimeSeries.csv};


\node[black, scale=0.9] at (axis cs: -100, 0.0) {\scriptsize Microwave};
\node[black, scale=0.9] at (axis cs: -100, 2.0) {\scriptsize Toaster\hphantom{vM}};
\node[black, scale=0.9] at (axis cs: -100, 4.0) {\scriptsize Kitchen\hphantom{vM}};

\pgfplotsinvokeforeach{0,60,128,151,170,421,451,481,502,721,788,813,834,901}{
    \draw [gray, thin] (axis cs: #1, -1.1) -- (axis cs: #1,-0.9);
}

\node [black, scale=0.5,rotate=270] at (axis cs: 0,-1.6) {\scriptsize 05:30};
\node [black, scale=0.5,rotate=270] at (axis cs: 60,-1.6) {\scriptsize 06:00};
\node [black, scale=0.5,rotate=270] at (axis cs: 128,-1.6) {\scriptsize 06:45};
\node [black, scale=0.5,rotate=270] at (axis cs: 151,-1.6) {\scriptsize 07:00};
\node [black, scale=0.5,rotate=270] at (axis cs: 168,-1.6) {\scriptsize 07:10};
\node [black, scale=0.5,rotate=270] at (axis cs: 421,-1.6) {\scriptsize 12:00};
\node [black, scale=0.5,rotate=270] at (axis cs: 451,-1.6) {\scriptsize 12:15};
\node [black, scale=0.5,rotate=270] at (axis cs: 481,-1.6) {\scriptsize 12:30};
\node [black, scale=0.5,rotate=270] at (axis cs: 502,-1.6) {\scriptsize 12:40};
\node [black, scale=0.5,rotate=270] at (axis cs: 721,-1.6) {\scriptsize 17:00};
\node [black, scale=0.5,rotate=270] at (axis cs: 788,-1.6) {\scriptsize 17:45};
\node [black, scale=0.5,rotate=270] at (axis cs: 813,-1.6) {\scriptsize 18:00};
\node [black, scale=0.5,rotate=270] at (axis cs: 834,-1.6) {\scriptsize 18:10};
\node [black, scale=0.5,rotate=270] at (axis cs: 901,-1.6) {\scriptsize 18:30};

% Microwave
\DrawON{149}{170}{1}
\DrawON{479}{500}{1}
\DrawON{810}{831}{1}

\DrawOFF{0}{148}{0}
\DrawOFF{171}{481}{0}
\DrawOFF{501}{811}{0}
\DrawOFF{832}{901}{0}

% Toaster
\DrawON{60}{128}{3}
\DrawON{421}{451}{3}
\DrawON{721}{788}{3}

\DrawOFF{0}{60}{2}
\DrawOFF{129}{421}{2}
\DrawOFF{451}{721}{2}
% \DrawOFF{811}{901}{2}
\DrawOFFSHIFT{789}{901}{2}{15}

% Kitchen
\DrawON{60}{151}{5}
\DrawON{721}{812}{5}

\DrawOFF{0}{60}{4}
\DrawOFFSHIFT{151}{721}{4}{50}
\DrawOFF{813}{901}{4}

\end{axis}
\end{tikzpicture}

==> data/tikz/timeSeries_new.tex <==
\begin{tikzpicture}
% sX,eX,Y
\newcommand{\DrawON}[3]{
	\draw [black,thin] (axis cs: #1, #3+0.15) -- (axis cs: #2, #3+0.15);
	\node [black, scale=0.5] at (axis cs: #1/2+#2/2, #3+0.45) {\small On};
}
% sX,eX,Y
\newcommand{\DrawOFF}[3]{
	\draw [black,thin] (axis cs: #1, #3-0.2) -- (axis cs: #2, #3-0.2);
	\node [black, scale=0.5] at (axis cs: #1/2+#2/2, #3-0.55) {\small Off};
}
% sX,eX,Y, Shift
\newcommand{\DrawOFFSHIFT}[4]{
	\draw [black,thin] (axis cs: #1, #3-0.2) -- (axis cs: #2, #3-0.2);
	\node [black, scale=0.5] at (axis cs: #1/2+#2/2+#4, #3-0.55) {\small Off};
}
\begin{axis}[
			 axis line style={draw=none},
             tick style={draw=none},
             ymin = -2.5, ymax = 6,
             xmin = -210, xmax = 950,
             xticklabels={0,,},
             yticklabels={,,},
             yscale=.35
             ]

\draw [black, thin, -latex] (axis cs: 0, -1) -- (axis cs: 950,-1) node [right] {};

\addplot [mark=none, color=cyan] table [x=x, y=microwave, col sep=comma] {data/tikz/newdataTimeSeries.csv};
\addplot [mark=none, color=orange] table [x=x, y=toaster, col sep=comma] {data/tikz/newdataTimeSeries.csv};
\addplot [mark=none, color=teal] table [x=x, y=kitchen, col sep=comma] {data/tikz/newdataTimeSeries.csv};


\node[black, scale=0.9] at (axis cs: -110, 0.0) {\footnotesize Microwave};
\node[black, scale=0.9] at (axis cs: -110, 2.0) {\footnotesize Toaster\hphantom{VM}};
\node[black, scale=0.9] at (axis cs: -110, 4.0) {\footnotesize Kitchen\hphantom{vM}};

\pgfplotsinvokeforeach{0,60,128,151,170,421,451,481,502,721,788,813,834,901}{
    \draw [gray, thin] (axis cs: #1, -1.15) -- (axis cs: #1,-0.85);
}

\node [black, scale=0.45,rotate=270] at (axis cs: 0,-1.9) {\footnotesize 05:30};
\node [black, scale=0.45,rotate=270] at (axis cs: 60,-1.9) {\footnotesize 06:00};
\node [black, scale=0.45,rotate=270] at (axis cs: 128,-1.9) {\footnotesize 06:45};
\node [black, scale=0.45,rotate=270] at (axis cs: 151,-1.9) {\footnotesize 07:00};
\node [black, scale=0.45,rotate=270] at (axis cs: 168,-1.9) {\footnotesize 07:10};
\node [black, scale=0.45,rotate=270] at (axis cs: 421,-1.9) {\footnotesize 12:00};
\node [black, scale=0.45,rotate=270] at (axis cs: 451,-1.9) {\footnotesize 12:15};
\node [black, scale=0.45,rotate=270] at (axis cs: 481,-1.9) {\footnotesize 12:30};
\node [black, scale=0.45,rotate=270] at (axis cs: 502,-1.9) {\footnotesize 12:40};
\node [black, scale=0.45,rotate=270] at (axis cs: 721,-1.9) {\footnotesize 17:00};
\node [black, scale=0.45,rotate=270] at (axis cs: 788,-1.9) {\footnotesize 17:45};
\node [black, scale=0.45,rotate=270] at (axis cs: 813,-1.9) {\footnotesize 18:00};
\node [black, scale=0.45,rotate=270] at (axis cs: 834,-1.9) {\footnotesize 18:10};
\node [black, scale=0.45,rotate=270] at (axis cs: 901,-1.9) {\footnotesize 18:30};

% Microwave
\DrawON{149}{170}{1}
\DrawON{479}{500}{1}
\DrawON{810}{831}{1}

\DrawOFF{0}{148}{0}
\DrawOFF{171}{481}{0}
\DrawOFF{501}{811}{0}
\DrawOFF{832}{901}{0}

% Toaster
\DrawON{60}{128}{3}
\DrawON{421}{451}{3}
\DrawON{721}{788}{3}

\DrawOFF{0}{60}{2}
\DrawOFF{129}{421}{2}
\DrawOFF{451}{721}{2}
% \DrawOFF{811}{901}{2}
\DrawOFFSHIFT{789}{901}{2}{25}

% Kitchen
\DrawON{60}{151}{5}
\DrawON{721}{812}{5}

\DrawOFF{0}{60}{4}
\DrawOFFSHIFT{151}{721}{4}{50}
\DrawOFF{813}{901}{4}

\end{axis}
\end{tikzpicture}

==> kFrequentAlg.tex <==
\subsubsection{Mining algorithm process}
\textbf{For k-event patterns}

\hspace{-0.15in}\textbf{Property 3.2} (Downward closure property of confidence \cite{omi}) Consider two temporal patterns $P^{'}$ and $P$. If $P^{'} \subseteq P$, then \textit{conf}($P^{'}$) $ \geq$ \textit{conf}($P$).

If this property is satisfied, we seek out all of k-event patterns between $n^{k-1}_i$ and $n^1_j$ (line 24). We now explain the way of looking for k-event patterns in function \textit{FindPatterns} (line 31). To mine k-event patterns, we find out the relations between the single events in $n^{k-1}_i$ and $n^1_j$. In this step, we use two properties for optimization: the \textit{transitive property} of the temporal relations and the \textit{property 4.4} of the all-confidence. Assuming that $n^{k-1}_i$ contains $\Sigma_i = \{a_1, a_2, ..., a_{k-1}\}$ and $n^1_j$ contains $\Sigma_j = \{b_1\}$. First, we find out the relations between $a_{k-1}$ and $b_1$ by accessing to the node at level 2 containing $\Sigma=\{a_{k-1}, b_1\}$ and getting 2-event patterns (line 34). If there is no any relations among them, we stop inspecting the temporal relations between $n^{k-1}_i$ and $n^1_j$ (line 39-40). Otherwise, by the \textit{transitive property}, there is a relation between each element in $\{a_1, a_2, ..., a_{k-2}\}$ and $b_1$, and we continue mining process. 

Throughout this process, if we do not find out a relation formed by $a_i \in \Sigma_i$ and $b_1$ that satisfies \textit{property 4.4}, then k-event patterns between $n^{k-1}_i$ and $n^1_j$ will be not established (lines 36-40). Applying \textit{transitive property} helps find relations among events quickly since looking for linearly relations among events does not ensure that it exists a relation between each element in $\{a_1, a_2, ..., a_{k-1}\}$ and $b_1$.
Finally, if there is at least one k-event pattern satisfying $\sigma$ and $\delta$, then a new node $n^k_m$ is created and its bitmap and maximum support value are inserted. Moreover, all of k-event patterns along with their TIIDs are also added to node $n^k_m$ (lines 25-29). The algorithm is stopped if we do not find out any the correlated k-event patterns.

\begin{lem}\textbf{Property 3.5} (Cross-support property of confidence \cite{ke2008correlated}) Given a pattern $P$, if there exist a sub-pattern $P_X \in P$ , such that $\frac{supp(P_X)}{\max_{1 \leq k \leq n}\{supp(E_k) \}} \leq \delta$ (where $n$ is size of $P$ and $E_k$ is a temporal event in $P$) then \textit{conf($P$)} $\leq \delta$.
\end{lem}

\begin{proof}
	\begin{equation}
	\small
	\text{\it{conf(P)}} = \frac{supp(P)}{\max_{1 \leq k \leq n}\{supp(E_k) \}} \leq \frac{supp(P_X)}{\max_{1 \leq k \leq n}\{supp(E_k) \}} \leq \delta
	\end{equation}
\end{proof}

\begin{lem} 
	The three temporal relations are mutual exclusive. 
\end{lem}
\begin{proof} Let two temporal events $E_1$ and $E_2$, and their corresponding instances, $e_1$ occurring during $[t_{s_1}, t_{e_1}]$ and $e_2$ occurring during $[t_{s_2}, t_{e_2}]$.
	There are three temporal relations that can happen between $E_1$ and $E_2$. Now we prove that if one of three relations happens then the remaining two relations do not happen. We consider the following cases.
	
	\hspace{-0.15in}\textit{Case 1:} We assume Follows($E_{1_{\triangleright e_1}}$, $E_{2_{\triangleright e_2}}$).
	
	\hspace{-0.15in}\textit{i.} We prove that Contains($E_{1_{\triangleright e_1}}$, $E_{2_{\triangleright e_2}}$) does not exist and vice versa.
	
	We have: Follows($E_{1_{\triangleright e_1}}$, $E_{2_{\triangleright e_2}})  \Rightarrow t_{e_1} \pm \epsilon \leq t_{s_2} $. 
	We also get: $t_{s_2} < t_{e_2}$.
	It follows: $t_{e_1} \pm \epsilon <  t_{e_2}$, and hence Contains($E_{1_{\triangleright e_1}}$, $E_{2_{\triangleright e_2}}$) condition is not satisfied $(t_{e_1} \pm \epsilon \geq  t_{e_2})$. Contrarily, Contains($E_{1_{\triangleright e_1}}$, $E_{2_{\triangleright e_2}}$) happens then Follows($E_{1_{\triangleright e_1}}$, $E_{2_{\triangleright e_2}}$) does not exist.
	
	\hspace{-0.15in}\textit{ii.} We prove that Overlaps($E_{1_{\triangleright e_1}}$, $E_{2_{\triangleright e_2}}$) does not exist and vice versa.
	
	We have: Follows($E_{1_{\triangleright e_1}}$, $E_{2_{\triangleright e_2}})  \Rightarrow t_{e_1} - t_{s_2} \leq \pm \epsilon$, thus Overlaps($E_{1_{\triangleright e_1}}$, $E_{2_{\triangleright e_2}}$) condition is not satisfied $(t_{e_1} - t_{s_2} \geq d_o \pm \epsilon)$. Contrarily, Overlaps($E_{1_{\triangleright e_1}}$, $E_{2_{\triangleright e_2}}$) happens then Follows($E_{1_{\triangleright e_1}}$, $E_{2_{\triangleright e_2}}$) does not exist.
	
	\hspace{-0.15in}\textit{Case 2:} We assume Contains($E_{1_{\triangleright e_1}}$, $E_{2_{\triangleright e_2}}$).
	
	We have: Contains$(E_{1_{\triangleright e_1}}$, $E_{2_{\triangleright e_2}}) \Rightarrow t_{e_1} \pm \epsilon \geq t_{e_2}$, thus Overlaps($E_{1_{\triangleright e_1}}$, $E_{2_{\triangleright e_2}}$) condition is not satisfied $(t_{e_1} \pm \epsilon < t_{e_2})$. Contrarily, Overlaps($E_{1_{\triangleright e_1}}$, $E_{2_{\triangleright e_2}}$) happens then Contains($E_{1_{\triangleright e_1}}$, $E_{2_{\triangleright e_2}}$) does not exist.
\end{proof}

\begin{lem}Let $\Re$ = \{Follow, Contain, Overlap\} be a set of relations and $I_E$ be a set of temporal events. $\Re$ is transitive on $I_E$.
	
	$ E_1, E_2, E_3 \in I_E; r_1, r_2 \in \Re: (r_1$ holds between $E_{1_{\triangleright e_1}}$  and  $E_{2_{\triangleright e_2}} ) \wedge (r_2$ holds between $E_{2_{\triangleright e_2}}$ and  $E_{3_{\triangleright e_3}} ) \Rightarrow \exists r_3 \in \Re \wedge (r_3$ holds between $E_{1_{\triangleright e_1}}$ and  $E_{3_{\triangleright e_3}} )$.
\end{lem}

\begin{proof}
	Let three temporal events $E_1$, $E_2$, $E_3$, and their corresponding instance, $e_1$ occurring during $[t_{s_1}, t_{e_1}]$, $e_2$ occurring during $[t_{s_2}, t_{e_2}]$, and $e_3$ occurring during $[t_{s_3}, t_{e_3}]$. 
	
	First, we show that $\forall r \in \Re: r$ holds between $E_{1_{\triangleright e_1}}$ and  $E_{2_{\triangleright e_2}} \Rightarrow t_{s_1} \leq t_{s_2}$.
	
	\begin{itemize}
		\item Consider r = ``Follow", then: $t_{e_1} \pm \epsilon \leq t_{s_2} \Rightarrow t_{e_1} \leq t_{s_2} \pm \epsilon$.
		We always get: $\epsilon < t_{e_1} - t_{s_1} \Rightarrow t_{e_1} > t_{s_1} + \epsilon$.
		Thus: $t_{s_1} + \epsilon < t_{s_2} \pm \epsilon \Rightarrow t_{s_1} < t_{s_2}$.
		\item Consider r = ``Contain": from the definition of Contains($E_{1_{\triangleright e_1}}, E_{2_{\triangleright e_2}}$) relation, we have $t_{s_1} \leq t_{s_2}$.
		\item Consider r = ``Overlap": from the definition of Overlaps($E_{1_{\triangleright e_1}}, E_{2_{\triangleright e_2}}$) relation, we have $t_{s_1} < t_{s_2}$.
	\end{itemize}
	
	Thus, we conclude: $\forall r \in \Re: r$ holds between $E_{1_{\triangleright e_1}}$ and  $E_{2_{\triangleright e_2}} \Rightarrow t_{s_1} \leq t_{s_2}$.
	
	We have: $r_1 \in \Re$, $r_1$ holds between $E_{1_{\triangleright e_1}}$ and  $E_{2_{\triangleright e_2}} \Rightarrow t_{s_1} \leq t_{s_2}$; $r_2 \in \Re$, $r_2$ holds between $E_{2_{\triangleright e_2}}$ and  $E_{3_{\triangleright e_3}} \Rightarrow t_{s_2} \leq t_{s_3}$. It follows: $t_{s_1} \leq t_{s_3}$, thus we conclude: it exists a relation between $E_1$ and $E_3$, i.e. $\exists r_3 \in \Re: r_3$ holds between $E_{1_{\triangleright e_1}}$ and  $E_{3_{\triangleright e_3}}$.
\end{proof}

Algorithm \ref{algorithmOpTPM} illustrates the mining process to build the patterns enumeration tree. First, database $\mathcal{D}_S$ is converted from $\mathcal{D}_T$ (line 1). Consequently, we search for the set of frequent single events at level 1 (lines 2-6). We compute the support value of every event \textit{e} in $\mathcal{D}_{S}$. If \textit{rel-supp}(\textit{e}) $>\sigma$ then \textit{e} is added to level 1 and its TIID and bitmap are also updated respectively.

%{\SetAlgoNoLine
%\SetNlSty{textbf}{}{:} %set number line in term of 1: , 2: and bold number
\SetNlSty{}{}{:} %set number line in term of 1: , 2:
\begin{algorithm}	
	\algsetup{linenosize=\tiny}
	\SetInd{0.5em}{0.5em}
	\small
	\DontPrintSemicolon
	\caption{The Temporal Patterns Mining OpCTPM}
	\label{algorithmOpTPM}
	
	\KwInput{A set of time series $\mathcal{D}_T$, minimum support threshold $\sigma$, minimum all-confidence threshold $\delta$}
	\KwOutput{The set of the correlated temporal patterns N(k)}
	
	convert $\mathcal{D}_T$ to $D_{Symbol}$ and $D_S$;\;
	\ForEach{\textit{transaction t} $\in \mathcal{D_S}$}{
		\ForEach{\textit{event e} $\in t$}{
			count e's support;\;
			$C1 \gets C1 \cup e$;
		}
	}
	$N(1) \gets \{e \in C1 | \textit{rel-supp}(e) \geq \sigma\}$;\;
	\ForEach{\textit{node} $n^1_i \in N(1)$}{
		%\ForEach{\textit{node} $n^1_j \in Siblings(n^1_i$)}{
		\ForEach{\textit{node} $n^1_j \in N(1)$)}{
			\If{$\textit{rel-supp}(n^1_i,n^1_j) \geq \sigma$}{
				\If{$\frac{supp(n^1_i)}{supp(n^1_j)} \geq \delta$ \textbf{and} $\frac{supp(n^1_j)}{supp(n^1_i)} \geq \delta $}{
					$\small \textit{patterns} \gets \small \text{Find2EventPattern}(n^1_i.\Sigma[0], n^1_j.\Sigma[0])$;\;
					\ForEach{\textit{pattern p} $\in$ \textit{patterns}}{
						\If{$\textit{rel-supp}(p) \geq \sigma$ \textbf{and} \textit{all-conf($p$)} $\geq \delta$}{
							$P^2(n^2_m) \gets P^2(n^2_m) \cup p$;\;
						}
					}
					$n^2_m \gets n^2_m \cup P^2(n^2_m)$;\;
					$N(2) \gets N(2) \cup n^2_m$;\;
				}
			}
		}
	}
	\BlankLine
	\While(\tcp*[h]{$k>2$}) {$N(k-1) \neq \emptyset$} {
		$N^{'}(1) \leftarrow \{n \in N(1) | n$ \textit{exists in} $N(k-1)\} $;\;
		\ForEach{\textit{node} $n^{k-1}_i \in N(k-1)$}{
			\ForEach{\textit{node} $n^1_j \in N^{'}(1)$}{
				\If{$\textit{rel-supp}(n^{k-1}_i,n^1_j) \geq \sigma$}{
					\If{$ \frac{supp(n^{k-1}_i)}{supp(n^1_j)} \geq \delta$ \textbf{and} $\frac{supp(n^1_j)}{supp(n^{k-1}_i)} \geq \delta$}{
						$max \gets max(supp(n^{k-1}_i),supp(n^1_j))$;\;
						$ patterns \gets \text{FindPatterns}(n^{k-1}_i, n^1_j, max)$;\;
						\ForEach{\textit{pattern} $p \in patterns$ }{
							\If{$\textit{rel-supp}(p) \geq \sigma$ \textbf{and} \textit{all-conf($p$)} $\geq \delta$}{
								$P^k(n^k_m) \gets P^k(n^k_m) \cup p$;\;
							}
						}			
						$n^k_m \gets n^k_m \cup P^k(n^k_m)$;\;
						$N(k) \gets N(k) \cup n^k_m$;
					}
				}
			}   		
		}
		$k = k + 1$;
	}
	\BlankLine
	\SetKwFunction{FMain}{FindPaterns}
	\SetKwProg{Fn}{Function}{}{}
	\Fn{\FMain{\textit{Node} $n^{k-1}_i$, \textit{Node} $n^1_j$, $max$}}{
		$P^k(n^k_i) \leftarrow P^{k-1}(n^{k-1}_i)$;\;    
		\For{$x \leftarrow k-1$ \KwTo $1$}{
			$ patterns \leftarrow \text{FindPatterns-Level2}(n^{k-1}_i.\Sigma[x], n^1_j.\Sigma[0])$;\;
			\textit{satisfied-patterns} $\leftarrow \emptyset$;\;
			\ForEach{\textit{pattern} $p \in patterns$}{
				%\If{$\textit{rel-supp}(p) \geq \sigma$}{
				%\If{$\frac{supp(p)}{max\{supp(n^{k-1}_i),supp(n^1_j)\}}\geq \delta$}{
				\If{$\frac{supp(p)}{max}\geq \delta$}{
					\textit{satisfied-patterns} $\leftarrow$ \textit{satisfied-patterns} $\cup  p$;
				}
				%}
			}
			\If{\textit{satisfied-patterns} $= \emptyset$}{
				\textbf{return} $\emptyset$; 
			}
			\Else{
				combine each pattern in \textit{satisfied-patterns} to each pattern in $P^k(n^k_i)$;
			}
		}
		\textbf{return} $P^k(n^k_i)$; 
	}
\end{algorithm}

\hspace{-0.15in}\textbf{Example 5.} Now we clarify the algorithm \ref{algorithmOpTPM} through the following example: consider database $\mathcal{D}_S$ in table \ref{tbl:SequenceDatabase}, given $\sigma=0.7$, $\delta = 0.7$. The patterns enumeration tree in Fig. \ref{fig:patternTree} is the result of this example. We scan $\mathcal{D}_S$ one time and filter the events by $\sigma$, we get $N(1)$=\{A[ON], A[OFF], B[ON], B[OFF], C[ON], C[OFF], D[OFF]\}. At level 2, each node at level 1 is considered with all nodes at level 1 for finding the correlated 2-event patterns. For instance, node A[ON] and node B[ON] are inspected. Since \textit{rel-supp}(A[ON],B[ON]) = 0.75 $\geq \sigma$, \textit{supp}(A[ON]) / \textit{supp}(B[ON]) = 1.33 $\geq \delta$ and \textit{supp}(B[ON]) / \textit{supp}(A[ON]) = 0.75 $\geq \delta$; so we continue looking for the relations between A[ON] and B[ON]. There is a relation among them ``A[ON]$\succcurlyeq$B[ON]" which occurs at temporal sequence ids \{1, 3, 4\}, and \textit{rel-supp}(A[ON]$\succcurlyeq$B[ON]) = 0.75 $\geq \sigma$, \textit{all-conf}(A[ON]$\succcurlyeq$B[ON]) = 0.75 $\geq \delta$; therefore, node \{A[ON], B[ON]\} is created and the pattern node ``A[ON]$\succcurlyeq$B[ON]" as well as its TIID are inserted into node \{A[ON], B[ON]\}. At level 3, each node at level 2 combines with all of nodes at level 1 which exist at level 2. Considering node \{A[ON], B[ON]\} and node \{C[ON]\}, we have $max=max$\{\textit{supp}(A[ON]),\textit{supp}(B[ON]),\textit{supp}(C[ON])\} = 4. Since \textit{rel-supp}(A[ON],B[ON],C[ON]) = 0.75 $\geq \sigma$, \textit{supp}(A[ON],B[ON]) / $max$ = 0.75 $\geq \delta$ and \textit{supp}(C[ON]) / $max$ = 0.75 $\geq \delta$, so we move on searching for the relations between A[ON], B[ON] and C[ON]. As the transitive property of the temporal relations, we first consider the relations between B[ON] and C[ON]. There is a relation B[ON]$\rightarrow$C[ON] and \textit{supp}(B[ON]$\rightarrow$C[ON]) / $max$ =0.75 $\geq \delta$, so there is a relation ``A[ON]$\succcurlyeq$B[ON], B[ON]$\rightarrow$C[ON]". Consequently, we take into account the relations between A[ON] and C[ON]. There is a relation A[ON] $\rightarrow$ C[ON] among them and \textit{supp}(A[ON]$\rightarrow$C[ON]) / $max$ = 0.75 $\geq \delta$. Thus, the node \{A[ON], B[ON]\} and the node \{C[ON]\} form one 3-event pattern ``A[ON]$\succcurlyeq$B[ON], B[ON]$\rightarrow$C[ON], A[ON] $\rightarrow$ C[ON]". The algorithm is stopped until not seeking out any k-event patterns.

\textbf{Time Complexity Analysis.} There are three steps in CTPM composing mining frequent single events, correlated 2-event patterns and correlated k-event patterns $(\text{k}>2$), so we analyse the time complexity for each step. First, to generate the frequent single events, we traverse $\mathcal{D}_S$, and update the support of each event in each temporal sequence of $\mathcal{D}_S$. Assuming that $w$ is the average temporal sequence width, the cost of the operation to find the frequent 1-event patterns requires $O(|\mathcal{D_S}| \cdot w)$. Consequently, to find the correlated 2-event patterns, each event in $N(1)$ is connected with all of events in $N(1)$; and the cost is $O(|N(1)^2|)$. Finally, to achieve the correlated k-event patterns $(\text{k}>2)$, each (k-1)-event patterns at $N(k-1)$ joins each 1-event pattern belonging $N^{'}(1)_{k-1}$, where  $N^{'}(1)_{k-1}$ is the single events belongs $N(1)$ and exists in $N(k-1)$. The cost of finding k-event patterns is $O(\sum_{k=3} |N(k-1)| \cdot |N^{'}(1)_{k-1}|)$. One process which is extremely important in OpCTPM is to find out the temporal relations among the temporal events beginning from level 2 in the patterns enumeration tree. This is based on k-event patterns' TIIDs. Assuming that $m$ is the TIID's average temporal sequence width and $t$ is the TIID's average size. The cost of searching for the relations among $k$ nodes is $t \cdot m^k$. Thus, the complexity of the OpCTPM is ${O\left(\scriptstyle{ |\mathcal{D_S}| \cdot w + |N(1)^2| \cdot t \cdot m^2) + \sum_{k=3} |N(k-1)| \cdot |N^{'}(1)_{k-1}| \cdot t \cdot m^k} \right)}$. However, in practice, due to applying the transitive property of the temporal relations the cost of our algorithm is much lower.

==> lemmaoverlappingsequence.tex <==
\hspace{-0.15in}\textbf{Lemma 1:} Let $\mathcal{D}_{Symbol}$ be a symbolic database, $\mathcal{D}_S$ be a temporal sequence database, $P$ be a temporal pattern in $\mathcal{D}_{Symbol}$, and $t_{max}$ be the maximal duration of $P$. $P$ exists in $\mathcal{D}_S$.
\begin{proof}
Assume that $P$ is formed by a temporal sequence $S=<e_1,..., e_n>$, where $e_1$ occurs during $[t_{s_1}, t_{e_1}]$ and $e_n$ occurs during $[t_{s_n}, t_{e_n}]$. We consider two cases.

Case 1: $P$ is only in a duration $T_i$ of $\mathcal{D}_{Symbol}$; therefore, $P$ is certainly in $\mathcal{D}_S$ after transformation.

Case 2: $P$ lies between two consecutive durations $T_i$ and $T_j$ in $\mathcal{D}_{Symbol}$. 

Without loss of generality, we assume that $T_i$ starts at $t_{s_i}$ and ends at $t_{e_i}$, $T_j$ starts at $t_{s_j}$ and ends at $t_{e_j}$. By the overlapping temporal sequences approach, to transform a temporal sequence at $T_i$ from $\mathcal{D}_{Symbol}$ to $\mathcal{D}_S$, event instances in $[t_{s_i}, t_{e_i}+ t_{max}]$ from $\mathcal{D}_{Symbol}$ are put into $\mathcal{D}_S$. Now we prove that $P$ is in $[t_{s_i}, t_{e_i}+ t_{max}]$.

By the property of the maximal duration of a temporal pattern, we get: $t_{e_n} - t_{s_1} \leq t_{max}$, hence $t_{e_n} \leq t_{s_1} + t_{max}$. Moreover, $t_{s_1}<t_{e_i}$ (P lies between $T_i$ and $T_j$). We deduce: $t_{e_n} < t_{e_i} + t_{max}$. And we also get: $t_{s_1} \geq t_{s_i}$ (P lies between $T_i$ and $T_j$). So, we have the conclusion: $P$ is in $[t_{s_i}, t_{e_i} + t_{max}]$; therefore, $P$ exists in $\mathcal{D}_S$.
\end{proof}


==> table/tableScalabilityAttributesPruned.tex <==
\begin{table*}[!t]
	\centering
		\caption{The Number of Pruned Attributes and the Accuracy of A-HTPGM}
		\vspace{-0.1in}
		\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
			\hline 
			\multirow{4}{*}{Supp. (\%)} & \multicolumn{16}{c|}{\bfseries Conf. (\%)} \\  
			\cline{2-17}  
			& \multicolumn{8}{c|}{\bfseries NIST} & \multicolumn{8}{c|}{\bfseries Smart City}
			\\  \cline{2-17}  
			& \multicolumn{4}{c|}{\bfseries Accuracy (\%)}  & \multicolumn{4}{c|}{\bfseries \# Patterns} & \multicolumn{4}{c|}{\bfseries Accuracy (\%)}  & \multicolumn{4}{c|}{\bfseries \# Patterns}    
			\\  \cline{2-17}  
			& {\bfseries 10} & {\bfseries 20} & {\bfseries 50}  & {\bfseries 80} & {\bfseries 10} & {\bfseries 20} & {\bfseries 50}    & {\bfseries 80} & {\bfseries 10} & {\bfseries 20} & {\bfseries 50}  & {\bfseries 80} & {\bfseries 10} & {\bfseries 20} & {\bfseries 50}    & {\bfseries 80} \\
			\hline
			10 & 72  & 79   & 95 & 100 & 3379003 & 1609573 & 152680 & 37351 & 71  & 90 & 100 & 100 & 1441723 & 1231025 & 102882 & 14021   \\  \hline			
			20 & 79  & 80   & 96  & 100 & 1596213 & 1557010 & 152680 & 36258  & 78  & 95 & 100  & 100 & 1291723 & 1201723 & 91032 & 7018 \\  \hline				
			50 & 95  & 96   & 100  & 100 & 197685 & 147775 & 146243 & 35997  & 95  & 100 & 100  & 100 & 595462 & 520467 & 60014 & 6219   \\  \hline					
			80 & 100  & 100   & 100  & 100 & 39821 & 35679 & 35679 & 28883 & 97  & 100 & 100  & 100 & 7366 & 7164 & 6546 & 6002  \\  \hline					
		\end{tabular}				
	\label{tbl:scalability_AttributePruned}
\end{table*}

==> table/tableSymbolDatabase.tex <==
\begin{table*}
	\begin{minipage}{.35\linewidth}
		\caption{A symbolic database $\mathcal{D}_{\text{SYB}}$}
		%\centering
		\resizebox{\textwidth}{7cm}{
			\begin{tabular}{|c|c|c|c|c|c|c|}
				\hline  \thead{Time} & \thead{K} & \thead{T} & \thead{M} & \thead{C} & \thead{I} & \thead{B} \\
				\hline
				\centering 10:00 & On & Off & Off & Off & Off & Off \\
				\centering 10:05 & On & On & Off & Off & Off & Off \\
				\centering 10:10 & On & On & Off & Off & Off & Off \\
				\centering 10:15 & On & On & Off & Off & Off & Off \\
				\centering 10:20 & Off & Off & On & On & Off & Off \\
				\centering 10:25 & Off & Off & On & On & Off & Off \\
				\centering 10:30 & Off & Off & On & On & Off & Off \\
				\centering 10:35 & On & On & Off & Off & Off & On \\
				\centering 10:40 & On & On & Off & Off & Off & On \\
				\hline
				\centering 10:45 & Off & Off & On & On & On & Off \\
				\centering 10:50 & Off & Off & On & On & On & Off \\
				\centering 10:55 & Off & On & On & Off & Off & Off \\
				\centering 11:00 & Off & On & Off & On & Off & Off \\
				\centering 11:05 & Off & Off & On & On & Off & Off \\
				\centering 11:10 & Off & Off & On & On & Off & Off \\
				\centering 11:15 & On & On & Off & Off & Off & Off \\
				\centering 11:20 & On & On & Off & Off & On & Off \\
				\centering 11:25 & On & On & Off & Off & On & Off \\
				\hline
				\centering 11:30 & Off & Off & On & On & Off & On \\
				\centering 11:35 & Off & Off & On & On & Off & On \\
				\centering 11:40 & Off & Off & Off & Off & Off & Off \\
				\centering 11:45 & Off & Off & On & On & Off & Off \\
				\centering 11:50 & On & On & On & On & Off & Off \\
				\centering 11:55 & On & On & Off & Off & Off & Off \\
				\centering 12:00 & On & On & Off & Off & Off & Off \\
				\centering 12:05 & Off & Off & On & On & Off & Off \\
				\centering 12:10 & Off & Off & On & On & Off & Off \\
				\hline
				\centering 12:15 & On & On & Off & Off & On & On \\
				\centering 12:20 & On & On & Off & Off & On & On \\
				\centering 12:25 & Off & Off & On & On & Off & Off \\
				\centering 12:30 & Off & Off & On & On & Off & Off \\
				\centering 12:35 & On & Off & On & On & Off & Off \\
				\centering 12:40 & On & On & Off & Off & On & Off \\
				\centering 12:45 & On & On & Off & Off & On & Off \\
				\centering 12:50 & Off & On & On & On & Off & On \\
				\centering 12:55 & Off & Off & On & On & Off & On \\
				\hline
			\end{tabular}
		}
		\label{tbl:SymbolDatabase}
	\end{minipage}%
%	\hspace{0.15in}
	\begin{minipage}{.65\linewidth}
		\centering
		\begin{minipage}{1.0\linewidth}	
			\caption{Temporal relations between events}
			\scriptsize
			\resizebox{\linewidth}{3.5cm}{
				\begin{tabular}{|m{0.18\columnwidth}| >{\centering\arraybackslash}m{0.65\columnwidth} |}
					\hline
					Follow relation: $E_{1_{\triangleright e_1}} \rightarrow E_{2_{\triangleright e_2}}$ & \begin{tikzpicture}
					
					\draw (0,0) -- node[below]{\textbf{e$_{1}$}} ++(0.7,0);
					\filldraw (0,0) circle (2pt)node[above]{\small t$_{s_1}$} ;
					\filldraw (0.7,0) circle (2pt)node[above ]{\small t$_{e_1}{\pm \epsilon}$};
					\filldraw (0.9,0) circle (2pt)node[below right]{\small t$_{s_2}$};
					\filldraw (2.3,0) circle (2pt)node[below]{\small t$_{e_2}$};
					\draw (0.9,0) -- node[above]{\textbf{e$_{2}$}} ++(1.4,0);
					
					%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
					\draw (3.5,0) -- node[below]{\textbf{e$_{1}$}} ++(0.7,0);
					\filldraw (3.5,0) circle (2pt)node[above]{\small t$_{s_1}$} ;
					\filldraw (4.2,0) circle (2pt)node[above]{\small t$_{e_1}{\pm \epsilon}$};
					\filldraw (4.7,0) circle (2pt)node[below right]{\small t$_{s_2}$};
					\filldraw (6.1,0) circle (2pt)node[below]{\small t$_{e_2}$};
					\draw (4.7,0) -- node[above]{\textbf{e$_{2}$}} ++(1.4,0);
				
					\node [align=center] at (3.3,-0.5) {\small t$_{e_1}{\pm \epsilon}$ $\le$ t$_{s_2}$};
					
					\end{tikzpicture}  \\ \hline
					
					Contain relation:\hspace{0.2in} $E_{1_{\triangleright e_1}} \succcurlyeq E_{2_{\triangleright e_2}}$ & 	
					\begin{tikzpicture}
					\draw (0,0) -- node[above]{\textbf{e$_1$}} ++(2.0,0);
					\filldraw (0,0) circle (2pt)node[above]{\small t$_{s_1}$} ;
					\filldraw (2,0) circle (2pt)node[above]{\small t$_{e_1}\pm \epsilon$};
					
					\draw (0,-0.4) -- node[above]{\textbf{e$_{2}$}} ++(2.0,0);
					\filldraw (0,-0.4) circle (2pt)node[below]{\small t$_{s_2}$} ;
					\filldraw (2,-0.4) circle (2pt)node[below]{\small t$_{e_2}$};
					
					
					\draw (3.5,0) -- node[above]{\textbf{e$_1$}} ++(2.1,0);
					\filldraw (3.5,0) circle (2pt)node[above]{\small t$_{s_1}$} ;
					\filldraw (5.6,0) circle (2pt)node[above]{\small t$_{e_1}\pm \epsilon$};	
					
					\draw (3.9,-0.4) -- node[above]{\textbf{e$_2$}} ++(1.4,0);
					\filldraw (3.9,-0.4) circle (2pt)node[below]{\small t$_{s_2}$} ;
					\filldraw (5.3,-0.4) circle (2pt)node[below]{\small t$_{e_2}$};	
					
					%%%%%%%%%%%%%%%
					%%%%%%%%%%%%%%%
					\draw (0,-1.3) -- node[above]{\textbf{e$_1$}} ++(2.0,0);
					%\filldraw (0,-2.0) circle (2pt)node[above]{\small t$_{s_1}\pm \epsilon$} ;
					\filldraw (0,-1.3) circle (2pt)node[above]{\small t$_{s_1}$} ;
					\filldraw (2.0,-1.3) circle (2pt)node[above]{\small t$_{e_1}\pm \epsilon$};
					
					\draw (-0,-1.7) -- node[above]{\textbf{e$_{2}$}} ++(1.5,0);
					\filldraw (0,-1.7) circle (2pt)node[below]{\small t$_{s_2}$} ;
					\filldraw (1.5,-1.7) circle (2pt)node[below]{\small t$_{e_2}$};
					
					%%\node [align=center] at (1,-5.0) {\small (t$_{s_{1}}{\pm \epsilon}$ = t$_{s_2}{\pm \epsilon}$) $\wedge$ \\ \hspace{0.2in} (t$_{e_1}{\pm \epsilon}$ $<$ t$_{e_2}{\pm \epsilon}$)};
					
					%%\node [align=center] at (1,-5.75) {\small ($\mid$ t$_{s_{2}}$ - t$_{s_1} \mid \le \epsilon$) $\wedge$ \\ \hspace{0.2in} ($\epsilon$ $\le \mid$ t$_{e_2}$ $-$ t$_{e_1} \mid$)};
					%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
					
					\draw (3.6,-1.3) -- node[above]{\textbf{e$_1$}} ++(2.0,0);
					%\filldraw (3.6,-2.0) circle (2pt)node[above]{t$_{s_1}\pm \epsilon$} ;
					\filldraw (3.6,-1.3) circle (2pt)node[above]{t$_{s_1}$} ;
					\filldraw (5.6,-1.3) circle (2pt)node[above]{t$_{e_1}\pm \epsilon$};
					
					\draw (4.1,-1.7) -- node[above]{\textbf{e$_{2}$}} ++(1.5,0);
					\filldraw (4.1,-1.7) circle (2pt)node[below]{t$_{s_2}$} ;
					\filldraw (5.6,-1.7) circle (2pt)node[below]{t$_{e_2}$};
					
					%%\node [align=center] at (2.25,-3.5) {\small (t$_{s_{1}}{\pm \epsilon}$ $\le$ t$_{s_2}$ $\vee$ t$_{s_{1}}$ $\le$ t$_{s_2}{\pm \epsilon}$) \\ \hspace{0.45in} $\wedge$ (t$_{e_1}{\pm \epsilon}$ $\ge$ t$_{e_2}$ $\vee$ t$_{e_1}$ $\ge$ t$_{e_2}{\pm \epsilon}$)};
					
					%\node [align=center] at (3.0,-3.5) {\small (t$_{s_{1}}{\pm \epsilon}$ $\le$ t$_{s_2}$)  $\wedge$ (t$_{e_1}{\pm \epsilon}$ $\ge$ t$_{e_2}$)};
					\node [align=center] at (3.0,-2.3) {\small (t$_{s_{1}} \le$ t$_{s_2}$)  $\wedge$ (t$_{e_1}{\pm \epsilon}$ $\ge$ t$_{e_2}$)};
					
					%%\node [align=center] at (4.5,-5.75) {\small ($\mid$ t$_{s_{1}}$ $-$ t$_{s_2} \mid \ge \epsilon$) $\wedge$\\ \hspace{0.2in} ( $\mid$ t$_{e_1}$ - t$_{e_2} \mid \le  \epsilon$)};
					
					\end{tikzpicture} \\ \hline
					Overlap relation: $E_{1_{\triangleright e_1}} \between E_{2_{\triangleright e_2}}$ & \begin{tikzpicture}
					
					\draw (0,0) -- node[above]{\textbf{e$_1$}} ++(2,0);
					%\filldraw (0,0) circle (2pt)node[above]{\small t$_{s_1}{\pm \epsilon}$} ;
					\filldraw (0,0) circle (2pt)node[above]{\small t$_{s_1}$} ;
					\filldraw (2,0) circle (2pt)node[above]{\small t$_{e_1}\pm \epsilon$};
					
					\draw (1,-0.6) -- node[above right]{\textbf{e$_{2}$}} ++(2.2,0);
					\filldraw (1,-0.6) circle (2pt)node[below]{\small t$_{s_2}$} ;
					\filldraw (3.2,-0.6) circle (2pt)node[below]{\small t$_{e_2}$};
					
					\draw[dashed] (1,0) -- (1,-0.6);
					\draw[dashed] (2,0) -- (2,-0.6);
					
					\draw[dashed,>=latex,thin,<->] (1,-0.325) -- node[above]{d$_{o}$} ++(1,0);
					
					\node [align=center] at (1.75,-1.2) {\small (t$_{s_1}<$ t$_{s_2}$) $\wedge$ (t$_{e_1}{\pm \epsilon}$ $<$ t$_{e_2}$) $\wedge$ 
						\small (t$_{e_1}$ $\textendash $ t$_{s_2}$ $\ge$ d${_o}{\pm \epsilon}$)};
					
					%\node [align=center] at (1.75,-2.5) {\small ($\epsilon \le \mid$ t$_{s_2}$ $-$ t$_{s_1}$) $\wedge$ ($\epsilon \le$ $\mid$ t$_{e_2}$ $-$ t$_{e_1}$) $\wedge$\\ 
					%\small ($\mid$ t$_{e_1}$ $\textendash$ t$_{s_2}$ $\mid) \ge$ d$_o$};
					
					\end{tikzpicture} \\
					\hline
			\end{tabular} }
			\label{tbl:relations}
			\vspace{0.1in}
		\end{minipage}
		\vspace{-0.1in}
		\begin{minipage}{1.0\linewidth}
			\caption{A temporal sequence database $\mathcal{D}_{\text{SEQ}}$}
%			\centering
			\resizebox{\columnwidth}{3cm}{
			\begin{tabular}{ |c|p{10.5cm}| }
				% \hline
				% \multicolumn{2}{|c|}{\textbf{Temporal sequence database}} \\
				\hline  \thead{ID} & \thead{Temporal sequences} \\
				\hline  
				1   &  (KOn,[10:00,10:15]), (KOff,[10:15,10:35]), (KOn,[10:35,10:40]), (TOff,[10:00,10:05]), (TOn,[10:05,10:15]), (TOff,[10:15,10:35]), (TOn,[10;35,10:40]), (MOff,[10:00,10:20]), (MOn,[10:20,10:30]), (MOff,[10:30,10:40]), (COff,[10:00,10:20]), (COn,[10:20,10:30]), (COff,[10:30,10:40]), (IOff,[10:00,10:40]), (BOff,[10:00,10:35]), (BOn,[10:35,10:40]) 
				\\
				\hline 
				2   &  (KOff,[10:45,11:15]), (KOn,[11:15,11:25]), (TOff,[10:45,10:55]), (TOn,[10:55,11:00]), (TOff,[11:00,11:15]), (TOn,[11:15,11:25]), (MOn,[10;45,10:55]), (MOff,[10:55,11:05]), (MOn,[11:05,11:10]), (MOff,[11:10,11:25]), (COn,[10:45,10:50]), (COff,[10:50,11:00]), (COn,[11:00,11:10]), (COff,[11:10,11:25]), (IOn,[10:45,10:50]), (IOff,[10:50,11:20]), (IOn,[11:20,11:25]), (BOff,[10:45,11:25])
				\\ 
				\hline 
				3   &  (KOff,[11:30,11:50]), (KOn,[11:50,12:00]), (KOff,[12:00,12:10]), (TOff,[11:30,11:50]), (TOn,[11:50,12:00]), (TOff,[12:00,12:10]), (MOn,[11:30,11:35]), (MOff,[11:35,11:45]), (MOn,[11:45,11:50]), (MOff,[11:50,12:05]), (MOn,[12:05,12:10]), (COn,[11:30,11:35]), (COff,[11:35,11:45]), (COn,[11:45,11:50]), (COff,[11:50,12:05]), (COn,[12:05,12:10]), (IOff,[11:30,12:10]), (BOn,[11:30,11:35]), (BOff,[11:35,12:10])
				\\
				\hline 
				4   &  (KOn,[12:15,12:20]), (KOff,[12:20,12:35]), (KOn,[12:35,12:45]), (KOff,[12:45,12:55]), (TOn,[12:15,12:20]), (TOff,[12:20,12:40]), (TOn,[12:40,12:50]), (TOff,[12:50,12:55]), (MOff,[12:15,12:25]), (MOn,[12:25,12:35]), (MOff,[12:35,12:50]), (MOn,[12:50,12:55]), (COff,[12:15,12:25]), (COn,[12:25,12:35]), (COff,[12:35,12:50]), (COn,[12:50,12:55]), (IOn,[12:15,12:20]), (IOff,[12:20,12:40]), (IOn,[12:40,12:45]), (IOff,[12:45,12:55]), (BOn,[12:15,12:20]), (BOff,[12:20,12:50]), (BOn,[12:50,12:55])
				\\
				\hline
			\end{tabular} }
			\label{tbl:SequenceDatabase}
		\end{minipage}
	\end{minipage} 
\end{table*}


==> tableQualitativeEvaluation.tex <==
\begin{table*}[!t]
	\vspace{-0.2in}
	\caption{Summary of Extracted Patterns}
	\centering
	\resizebox{\textwidth}{!}{
		\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
			\hline 
			\multirow{2}{*}{Support (\%)}  & \multicolumn{16}{c|}{\bfseries Confidence (\%)}
			\\  \cline{2-17}  
			& \multicolumn{4}{c|}{\bfseries NIST}  & \multicolumn{4}{c|}{\bfseries UKDALE}   & \multicolumn{4}{c|}{\bfseries DataPort} & \multicolumn{4}{c|}{\bfseries Smart City}
			\\  \hline
			& {\bfseries 20} & {\bfseries 40}  & {\bfseries 60}  & {\bfseries 80} & {\bfseries 20} & {\bfseries 40}  & {\bfseries 60}  & {\bfseries 80} & {\bfseries 20} & {\bfseries 40}  & {\bfseries 60}  & {\bfseries 80} & {\bfseries 20} & {\bfseries 40}  & {\bfseries 60}  & {\bfseries 80} \\
			\hline
			\centering 20  & 519,316 & 378,896 & 69,951 & 28,912 & 126,490 & 39,629 & 10,562 & 4,231 & 310,713 & 200,179 & 11,074 & 5,012 & 1,201,723 & 1,001,354 & 121,140 & 7,164   \\  \hline
			\centering 40  & 96,952 & 96,952 & 46,793 & 14,193 & 46,193 & 26,172 & 8,240 & 4,129 & 201,561 & 140,984 & 8,928 & 4,813 & 91,241 & 90,198 & 76,014 & 6,891  \\  \hline
			\centering 60  & 29,955 & 29,955 & 29,955 & 9,608 & 11,247 & 6,221 & 5,392 & 3,921 & 9,781 & 7,229 & 6,582 & 3,827 & 13,126 & 8,712 & 6,286 & 6,140  \\  \hline
			\centering 80  & 3,568 & 3,568 & 3,568 & 3,568 & 4,832 & 4,321 & 3,251 & 3,251 & 5,492 & 4,825 & 3,981 & 3,370 & 7,018 & 6,872 & 6,002 & 6,002  \\  \hline
		\end{tabular}
	}
	\label{tbl:numberextractedPatterns}
	%\vspace{-0.05in}
\end{table*}

%\begin{table}
%	\caption{Generated patterns of \ref{text:datasetElectricMinute}.}
%	\centering
%	\resizebox{\columnwidth}{!}{
%		\begin{tabular}{|c|c|c|c|c|}
%			\hline
%			\multicolumn{5}{|c|}{\bfseries Patterns generated for \ref{text:datasetElectricMinute}}    
%			\\  \hline
%			{}  & {\bfseries 20\% Conf.} & {\bfseries 40\% Conf.}  & {\bfseries 60\% Conf.}  & {\bfseries 80\% Conf.} \\
%			\hline
%			\centering 20\% support & 519,316 & 378,896 & 69,951 & 28,912  \\  \hline
%			\centering 40\% support & 96,952 & 96,952 & 46,793 & 14,193  \\  \hline
%			\centering 60\% support & 29,955 & 29,955 & 29,955 & 9,608  \\  \hline
%			\centering 80\% support & 3,568 & 3,568 & 3,568 & 3,568  \\  \hline
%		\end{tabular}
%	}
%	\label{tbl:numberPatternsNIST}
%\end{table}

%\begin{table}
%	\caption{Generated patterns of \ref{text:datasetUKDALE}.}
%	\centering
%	\resizebox{\columnwidth}{!}{
%		\begin{tabular}{|c|c|c|c|c|}
%			\hline
%			\multicolumn{5}{|c|}{\bfseries Patterns generated for \ref{text:datasetUKDALE}}    
%			\\  \hline
%			{}  & {\bfseries 20\% Conf.} & {\bfseries 40\% Conf.}  & {\bfseries 60\% Conf.}  & {\bfseries 80\% Conf.} \\
%			\hline
%			\centering 20\% support & 126490 & 39629 & 10562 & 4231  \\  \hline
%			\centering 40\% support & 46193 & 26172 & 8240 & 4129  \\  \hline
%			\centering 60\% support & 11247 & 6221 & 5392 & 3921  \\  \hline
%			\centering 80\% support & 4832 & 4321 & 3251 & 3251  \\  \hline
%		\end{tabular}
%	}
%	\label{tbl:numberPatternsUKDALE}
%\end{table}
%
%\begin{table}
%	\caption{Generated patterns of \ref{text:datasetDataport}.}
%	\centering
%	\resizebox{\columnwidth}{!}{
%		\begin{tabular}{|c|c|c|c|c|}
%			\hline
%			\multicolumn{5}{|c|}{\bfseries Patterns generated for \ref{text:datasetDataport}}    
%			\\  \hline
%			{}  & {\bfseries 20\% Conf.} & {\bfseries 40\% Conf.}  & {\bfseries 60\% Conf.}  & {\bfseries 80\% Conf.} \\
%			\hline
%			\centering 20\% support & 310713 & 200179 & 11074 & 5012  \\  \hline
%			\centering 40\% support & 201561 & 140984 & 8928 & 4813  \\  \hline
%			\centering 60\% support & 9781 & 7229 & 6582 & 3827  \\  \hline
%			\centering 80\% support & 5492 & 4825 & 3981 & 3370  \\  \hline
%		\end{tabular}
%	}
%	\label{tbl:numberPatternsPecanStreet}
%\end{table}

%\begin{table}
%	\caption{Generated patterns of \ref{text:datasetMotorist}.}
%	\centering
%	\resizebox{\columnwidth}{!}{
%		\begin{tabular}{|c|c|c|c|c|}
%			\hline
%			\multicolumn{5}{|c|}{\bfseries Patterns generated for \ref{text:datasetMotorist}}    
%			\\  \hline
%			{}  & {\bfseries 20\% Conf.} & {\bfseries 40\% Conf.}  & {\bfseries 60\% Conf.}  & {\bfseries 80\% Conf.} \\
%			\hline
%			\centering 20\% support & 1201723 & 1001354 & 121140 & 7164  \\  \hline
%			\centering 40\% support & 91241 & 90198 & 76014 & 6891  \\  \hline
%			\centering 60\% support & 13126 & 8712 & 6286 & 6140  \\  \hline
%			\centering 80\% support & 7018 & 6872 & 6002 & 6002  \\  \hline
%		\end{tabular}
%	}
%	\label{tbl:numberPatternsSmartCity}
%\end{table}

\begin{table*}[!t]
	%\vspace{-0.1in}
	\caption{Summary of Interesting Patterns}
	\centering
	\resizebox{\textwidth}{!}{
		\begin{tabular}{ |p{16cm}|p{0.5cm}|p{0.5cm}| }
			\hline  \thead{Patterns} & \thead{Supp. \%} & \thead{Conf. \%}\\
			\hline  
			(P1) ([05:58, 08:24] First Floor Lights On) $\succcurlyeq$ ([05:58, 06:59] Upstairs Bathroom Lights On) $\succcurlyeq$ ([05:59, 06:06] Microwave On) &  20 & 30  \\
			\hline
			(P2) ([06:00, 07:01] Upstairs Bathroom Lights On) $\succcurlyeq$ ([06:40,  06:46] Upstairs Bathroom Plugs On) &  30 & 20   \\
			\hline 
			(P3) ([18:00, 18:30] Lights Dining Room On) $\rightarrow$ ([18:31, 20:16] Children Room Plugs On) $\between$ ([19:00, 22:31] Lights Living Room On) & 20  &  20 \\
			\hline
			(P4) ([15:59, 16:05] Hallway Lights On) $\rightarrow$ ([17:58, 18:29] Kitchen Lights On $\succcurlyeq$ ([18:00, 18:18] Plug In Kitchen On) $\succcurlyeq$ ([18:08, 18:15] Microwave On) &  80 & 60 \\
			\hline
			(P5) ([06:02, 06:19] Kitchen Lights On) $\rightarrow$ ([06:05, 06:12] Microwave On) $\between$ ([06:09, 06:11] Kettle On) & 20 & 5\\
			\hline 
			(P6) ([05:58,08:24] First Floor Lights On) $\succcurlyeq$ ([05:58,06:59] Upstairs Bathroom Lights On) $\succcurlyeq$ ([05:59, 06:06] Microwave On)   &  20 & 30
			\\ \hline 
			(P7) ([06:00,07:01] Upstairs Bathroom Lights On) $\succcurlyeq$ ([06:40,06:46] Upstairs Bathroom Plugs On)   &  30 & 20
			\\ \hline 
			(P8) ([18:10,18:15] Kitchen App) $\rightarrow$ ([18:15,19:00] Lights Plugs) $\succcurlyeq$ ([18:20,18:25] Microwave) $\rightarrow$ ([18:25,18:55] Cooktop) $\rightarrow$ [(19:30,20:20) Clothes Dryer)   &  5 & 50
			\\ \hline 
			(P9) ([16:45, 17:30] Clothes Washer) $\rightarrow$ ([17:40,18:55] Clothes Dryer) $\rightarrow$ ([19:05, 20:10] Dining Room)  $\succcurlyeq$ ([19:10, 19:30] Cooktop)
			&  10 & 30
			\\ \hline 
			(P10) ([06:10, 07:00] Kitchen Lights) $\succcurlyeq$ ([06:10, 06:15] Kettle) $\rightarrow$ ([06:30, 06:40] Toaster) $\rightarrow$ ([06:45, 06:48] Microwave)   &  25 & 40
			\\ \hline 
			(P11) ([18:00, 18:25] Kitchen Lights) $\succcurlyeq$ ([18:00, 18:05] Kettle) $\rightarrow$ ([18:05, 18:10] Microwave) $\rightarrow$ ([19:35, 20:50] Washing Machine)   &  20 & 40
			\\ \specialrule{1.5pt}{1pt}{1pt}
			(P12) ([13:10, 22:35] Heavy Rain) $\succcurlyeq$ ([14:00, 22:35] Unclear Visibility) $\succcurlyeq$ ([15:00, 20:55] Overcast Cloudiness) $\rightarrow$ ([21:00, 21:55] High Motorist Collision)   &  5 & 30
			\\ \hline 
			(P13) ([19:00, 21:50] Unclear Extremely Visibility) $\succcurlyeq$ ([19:00, 21:50] High Snow) $\succcurlyeq$ ([20:00, 20:55] High Motorist Collision)   &  30 & 45 \\
			\hline
			(P14) Very Strong Wind $\rightarrow$ High Motorist Injury & 5 & 40 \\
			\hline
			(P15) Frost Temperature $\rightarrow$ Medium Cyclist Injury & 5& 20 \\
			\hline
			(P16) Strong Wind $\rightarrow$ High Pedestrian Killed & 4 & 30\\
			\hline
			(P17) Strong Wind $\rightarrow$ High Motorist Killed  & 4 & 10\\
			\hline 
		\end{tabular} 
	}
	\label{tbl:interestingPatterns}
	\vspace{-0.15in}
\end{table*}

%P1 shows the living pattern of the residents. Here, we can see one of the residents turns the light upstairs on in early morning, and goes to the bathroom. Then, within a minute, the microwave is turned on. This could imply that there might be more than one person living in the house, where one is in the bathroom, and another is downstairs preparing breakfast. %This pattern is found $81$ times in the dataset with similar timespan. 

%In P2, we can see the light in the bathroom is turned on for an hour. This could hint that the person might be showering. During this time, the plug in the bathroom is used for $6$ minutes. This happens after the bathroom light has been active for $40$ minutes. This could indicate that the person is using a hair dryer after the shower. %This pattern occurs $129$ times. 
%The pattern P3 also indicates the living habits of the residents. Here, the lights downstairs in the dining room are on, but then off at 18:30, after which the plugs in children bedroom are on. This could be a bed lamp, where the parents are spending time with their children. After for about $30$ minutes, the lights are on in the living room, which might indicate that the parents are spending their times downstairs, before going to bed around 22:31, when the lights turn off. %This rule occurs $63$ times. % in total. %This rule happens about every other day.

%In P4, we see the lights in the hall entry is on at 15:59, which could indicate that the residents have arrived home. They proceed to move around the house and the family begins to prepare dinner at 18:00 by activating the light and the apparatus inserted into the kitchen plugs, together with the microwave a few minutes later. This pattern is seen almost daily. Other patterns such as P5 show how the residents interact with the appliances.   

%\textit{The Weather and Vehicle Collision datasets:}
%Unsurprisingly, in these datasets, we found that a majority of extracted patterns are related to normal weather conditions and collision situations. For example, the crashes are less severe in normal weather conditions. This is one of the patterns: \textit{(Medium Temperature - Low Wind Speed - High Visibility - No Rain - No Thunder - No Tornado) $\rightarrow$ (No Injury - No Death)}. Such patterns occur frequently with very high support, e.g., 80\% of the time. However, these patterns do not reveal interesting information. 

%To look for more useful patterns, we pay attention to the extreme weather events, which happen rarely with low support. We found that extreme weather conditions are likely associated with higher number of collisions, such as the patterns P6, P7, P8, and P9. 

==> tableSymbolDatabase.tex <==
%An example of the symbolic database $\mathcal{D}_{\text{SYB}}$ is shown in Table \ref{tbl:SymbolDatabase}. There are $6$ time series representing the energy usage of $6$ electrical appliances: \{Stove, Toaster, Microwave, Clothes Washer, Dryer, Iron\}. For brevity, we name the appliances respectively as \{S, T, M, W, D, I\}. All appliances have the same alphabet $\Sigma$ = \{On, Off\}. 

%, and the symbolic database $\mathcal{D}_{\text{SYB}}$ is obtained by transforming each time series into a sequence of symbols, as in Table \ref{tbl:SymbolDatabase}. %mapping each raw value of the time series into the states On/Off of each appliance.%And table \ref{tbl:SequenceDatabase} is the result of converting data from $\mathcal{D}_{Symbol}$ to $\mathcal{D}_S$.

%\input{table/tableSymbolDatabase_SmallerSpace.tex}

%\input{table/tableSymbolDatabase.tex}

%Old table
%\begin{table*}
%	\begin{minipage}{.4\linewidth}
%		\vspace*{-0.15in}
%		\caption{A symbolic database $\mathcal{D}_{\text{SYB}}$}
%		\resizebox{1.0\columnwidth}{!}{
%			\small
%			\begin{tabular}{|c|c|c|c|c|c|c|}
%				\hline  \thead{Time} & \thead{K} & \thead{T} & \thead{M} & \thead{C} & \thead{I} & \thead{B} \\
%				\hline
%				\centering 10:00 & On & Off & Off & Off & Off & Off \\
%				\centering 10:05 & On & On & Off & Off & Off & Off \\
%				\centering 10:10 & On & On & Off & Off & Off & Off \\
%				\centering 10:15 & On & On & Off & Off & Off & Off \\
%				\centering 10:20 & Off & Off & On & On & Off & Off \\
%				\centering 10:25 & Off & Off & On & On & Off & Off \\
%				\centering 10:30 & Off & Off & On & On & Off & Off \\
%				\centering 10:35 & On & On & Off & Off & Off & On \\
%				\centering 10:40 & On & On & Off & Off & Off & On \\
%				\hline
%				\centering 10:45 & Off & Off & On & On & On & Off \\
%				\centering 10:50 & Off & Off & On & On & On & Off \\
%				\centering 10:55 & Off & On & On & Off & Off & Off \\
%				\centering 11:00 & Off & On & Off & On & Off & Off \\
%				\centering 11:05 & Off & Off & On & On & Off & Off \\
%				\centering 11:10 & Off & Off & On & On & Off & Off \\
%				\centering 11:15 & On & On & Off & Off & Off & Off \\
%				\centering 11:20 & On & On & Off & Off & On & Off \\
%				\centering 11:25 & On & On & Off & Off & On & Off \\
%				\hline
%				\centering 11:30 & Off & Off & On & On & Off & On \\
%				\centering 11:35 & Off & Off & On & On & Off & On \\
%				\centering 11:40 & Off & Off & Off & Off & Off & Off \\
%				\centering 11:45 & Off & Off & On & On & Off & Off \\
%				\centering 11:50 & On & On & On & On & Off & Off \\
%				\centering 11:55 & On & On & Off & Off & Off & Off \\
%				\centering 12:00 & On & On & Off & Off & Off & Off \\
%				\centering 12:05 & Off & Off & On & On & Off & Off \\
%				\centering 12:10 & Off & Off & On & On & Off & Off \\
%				\hline
%				\centering 12:15 & On & On & Off & Off & On & On \\
%				\centering 12:20 & On & On & Off & Off & On & On \\
%				\centering 12:25 & Off & Off & On & On & Off & Off \\
%				\centering 12:30 & Off & Off & On & On & Off & Off \\
%				\centering 12:35 & On & Off & On & On & Off & Off \\
%				\centering 12:40 & On & On & Off & Off & On & Off \\
%				\centering 12:45 & On & On & Off & Off & On & Off \\
%				\centering 12:50 & Off & On & On & On & Off & On \\
%				\centering 12:55 & Off & Off & On & On & Off & On \\
%				\hline
%			\end{tabular}
%		}
%		\label{tbl:SymbolDatabase}
%	\end{minipage}%
%	\hspace{0.15in}
%	\begin{minipage}{.6\linewidth}
%		\centering
%		\begin{minipage}{1.0\linewidth}	
%			\caption{Temporal relations between events}
%			\centering
%			\scriptsize
%			\hspace*{-0.5in}\\
%			\resizebox{\columnwidth}{!}{
%				\begin{tabular}{|m{0.18\columnwidth}| m{0.65\columnwidth} |}
%					\hline
%					\thead{Relation} & \thead{} \\
%					\hline
%					Follow relation: $E_{1_{\triangleright e_1}} \rightarrow E_{2_{\triangleright e_2}}$ & \begin{tikzpicture}
					
%					\draw (0,0) -- node[below]{\textbf{e$_{1}$}} ++(0.7,0);
%					\filldraw (0,0) circle (2pt)node[above]{\small t$_{s_1}$} ;
%					\filldraw (0.7,0) circle (2pt)node[above ]{\small t$_{e_1}{\pm \epsilon}$};
%					
%					\filldraw (0.9,0) circle (2pt)node[below right]{\small t$_{s_2}$};
%					\filldraw (2.3,0) circle (2pt)node[below]{\small t$_{e_2}$};
%					\draw (0.9,0) -- node[above]{\textbf{e$_{2}$}} ++(1.4,0);
					
					%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%					\draw (3.5,0) -- node[below]{\textbf{e$_{1}$}} ++(0.7,0);
%					\filldraw (3.5,0) circle (2pt)node[above]{\small t$_{s_1}$} ;
%					\filldraw (4.2,0) circle (2pt)node[above]{\small t$_{e_1}{\pm \epsilon}$};
					
%					\filldraw (4.7,0) circle (2pt)node[below right]{\small t$_{s_2}$};
%					\filldraw (6.1,0) circle (2pt)node[below]{\small t$_{e_2}$};
%					\draw (4.7,0) -- node[above]{\textbf{e$_{2}$}} ++(1.4,0);
					
%					\node [align=center] at (3.5,-0.7) {\small t$_{e_1}{\pm \epsilon}$ $\le$ t$_{s_2}$};
%					\end{tikzpicture}  \\ \hline
					
%					Contain relation:\hspace{0.2in} $E_{1_{\triangleright e_1}} \succcurlyeq E_{2_{\triangleright e_2}}$ & 	\begin{tikzpicture}
%					\draw (0,0) -- node[above]{\textbf{e$_1$}} ++(2.0,0);
%					\filldraw (0,0) circle (2pt)node[above]{\small t$_{s_1}$} ;
%					\filldraw (2,0) circle (2pt)node[above]{\small t$_{e_1}\pm \epsilon$};
					
%					\draw (0,-0.5) -- node[above]{\textbf{e$_{2}$}} ++(2.0,0);
%					\filldraw (0,-0.5) circle (2pt)node[below]{\small t$_{s_2}$} ;
%					\filldraw (2,-0.5) circle (2pt)node[below]{\small t$_{e_2}$};
	
					%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
					
%					\draw (3.5,0) -- node[above]{\textbf{e$_1$}} ++(2.1,0);
%					\filldraw (3.5,0) circle (2pt)node[above]{\small t$_{s_1}$} ;
%					\filldraw (5.6,0) circle (2pt)node[above]{\small t$_{e_1}\pm \epsilon$};	
					
%					\draw (3.9,-0.5) -- node[above]{\textbf{e$_2$}} ++(1.4,0);
%					\filldraw (3.9,-0.5) circle (2pt)node[below]{\small t$_{s_2}$} ;
%					\filldraw (5.3,-0.5) circle (2pt)node[below]{\small t$_{e_2}$};	
					
					%%%%%%%%%%%%%%%
					%%%%%%%%%%%%%%%
%					\draw (0,-1.5) -- node[above]{\textbf{e$_1$}} ++(2.0,0);
%					\filldraw (0,-1.5) circle (2pt)node[above]{\small t$_{s_1}$} ;
%					\filldraw (2.0,-1.5) circle (2pt)node[above]{\small t$_{e_1}\pm \epsilon$};
					
%					\draw (-0,-2) -- node[above]{\textbf{e$_{2}$}} ++(1.5,0);
%					\filldraw (0,-2) circle (2pt)node[below]{\small t$_{s_2}$} ;
%					\filldraw (1.5,-2) circle (2pt)node[below]{\small t$_{e_2}$};
					
					%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
					
%					\draw (3.6,-1.5) -- node[above]{\textbf{e$_1$}} ++(2.0,0);
%					\filldraw (3.6,-1.5) circle (2pt)node[above]{t$_{s_1}$} ;
%					\filldraw (5.6,-1.5) circle (2pt)node[above]{t$_{e_1}\pm \epsilon$};
					
%					\draw (4.1,-2) -- node[above]{\textbf{e$_{2}$}} ++(1.5,0);
%					\filldraw (4.1,-2) circle (2pt)node[below]{t$_{s_2}$} ;
%					\filldraw (5.6,-2) circle (2pt)node[below]{t$_{e_2}$};
					
%					\node [align=center] at (3.0,-2.7) {\small (t$_{s_{1}} \le$ t$_{s_2}$)  $\wedge$ (t$_{e_1}{\pm \epsilon}$ $\ge$ t$_{e_2}$)};
					
%					\end{tikzpicture} \\ \hline
%					Overlap relation: $E_{1_{\triangleright e_1}} \between E_{2_{\triangleright e_2}}$ & \begin{tikzpicture}
					
%					\draw (0,0) -- node[above]{\textbf{e$_1$}} ++(2,0);
%					\filldraw (0,0) circle (2pt)node[above]{\small t$_{s_1}$} ;
%					\filldraw (2,0) circle (2pt)node[above]{\small t$_{e_1}\pm \epsilon$};
					
%					\draw (1,-0.75) -- node[above right]{\textbf{e$_{2}$}} ++(2.0,0);
%					\filldraw (1,-0.75) circle (2pt)node[below]{\small t$_{s_2}$} ;
%					\filldraw (3,-0.75) circle (2pt)node[below]{\small t$_{e_2}$};
					
%					\draw[dashed] (1,0) -- (1,-0.75);
%					\draw[dashed] (2,0) -- (2,-0.75);
					
%					\draw[dashed,>=latex,thin,<->] (1,-0.325) -- node[above]{d$_{o}$} ++(1,0);
					
%					\node [align=center] at (1.75,-1.45) {\small (t$_{s_1}<$ t$_{s_2}$) $\wedge$ (t$_{e_1}{\pm \epsilon}$ $<$ t$_{e_2}$) $\wedge$ 
%						\small (t$_{e_1}$ $\textendash $ t$_{s_2}$ $\ge$ d${_o}{\pm \epsilon}$)};
					
%					\end{tikzpicture} \\
%					\hline
%			\end{tabular} }
%			\label{tbl:relations}
%			\vspace{0.1in}
%		\end{minipage}
%		\vspace{-0.1in}
%		\begin{minipage}{1.0\linewidth}
%			\caption{A temporal sequence database $\mathcal{D}_{\text{SEQ}}$}
%			\centering
%			\resizebox{\columnwidth}{!}{
%			\begin{tabular}{ |c|p{10.5cm}| }
%				\hline  \thead{ID} & \thead{Temporal sequences} \\
%				\hline  
%				1   &  (KOn,[10:00,10:15]), (KOff,[10:15,10:35]), (KOn,[10:35,10:40]), (TOff,[10:00,10:05]), (TOn,[10:05,10:15]), (TOff,[10:15,10:35]), (TOn,[10;35,10:40]), (MOff,[10:00,10:20]), (MOn,[10:20,10:30]), (MOff,[10:30,10:40]), (COff,[10:00,10:20]), (COn,[10:20,10:30]), (COff,[10:30,10:40]), (IOff,[10:00,10:40]), (BOff,[10:00,10:35]), (BOn,[10:35,10:40]) 
%				\\
%				\hline 
%				2   &  (KOff,[10:45,11:15]), (KOn,[11:15,11:25]), (TOff,[10:45,10:55]), (TOn,[10:55,11:00]), (TOff,[11:00,11:15]), (TOn,[11:15,11:25]), (MOn,[10;45,10:55]), (MOff,[10:55,11:05]), (MOn,[11:05,11:10]), (MOff,[11:10,11:25]), (COn,[10:45,10:50]), (COff,[10:50,11:00]), (COn,[11:00,11:10]), (COff,[11:10,11:25]), (IOn,[10:45,10:50]), (IOff,[10:50,11:20]), (IOn,[11:20,11:25]), (BOff,[10:45,11:25])
%				\\ 
%				\hline 
%				3   &  (KOff,[11:30,11:50]), (KOn,[11:50,12:00]), (KOff,[12:00,12:10]), (TOff,[11:30,11:50]), (TOn,[11:50,12:00]), (TOff,[12:00,12:10]), (MOn,[11:30,11:35]), (MOff,[11:35,11:45]), (MOn,[11:45,11:50]), (MOff,[11:50,12:05]), (MOn,[12:05,12:10]), (COn,[11:30,11:35]), (COff,[11:35,11:45]), (COn,[11:45,11:50]), (COff,[11:50,12:05]), (COn,[12:05,12:10]), (IOff,[11:30,12:10]), (BOn,[11:30,11:35]), (BOff,[11:35,12:10])
%				\\
%				\hline 
%				4   &  (KOn,[12:15,12:20]), (KOff,[12:20,12:35]), (KOn,[12:35,12:45]), (KOff,[12:45,12:55]), (TOn,[12:15,12:20]), (TOff,[12:20,12:40]), (TOn,[12:40,12:50]), (TOff,[12:50,12:55]), (MOff,[12:15,12:25]), (MOn,[12:25,12:35]), (MOff,[12:35,12:50]), (MOn,[12:50,12:55]), (COff,[12:15,12:25]), (COn,[12:25,12:35]), (COff,[12:35,12:50]), (COn,[12:50,12:55]), (IOn,[12:15,12:20]), (IOff,[12:20,12:40]), (IOn,[12:40,12:45]), (IOff,[12:45,12:55]), (BOn,[12:15,12:20]), (BOff,[12:20,12:50]), (BOn,[12:50,12:55])
%				\\
%				\hline
%			\end{tabular} }
%			\label{tbl:SequenceDatabase}
%		\end{minipage}
%	\end{minipage} 
%\end{table*}


==> tableSymbolDatabase_bk.tex <==
Table \ref{tbl:SymbolDatabase} is an example of a symbolic database $\mathcal{D}_{Symbol}$, which is transformed from a set of time series data of energy consumption. The data is observed during four days and the appliances' energy usage is recorded from 18:00 to 20:00 for each day. And table \ref{tbl:SequenceDatabase} is the result of converting data from $\mathcal{D}_{Symbol}$ to $\mathcal{D}_S$.

\begin{table}
\caption{A symbolic database $\mathcal{D}_{Symbol}$}
\centering
\begin{tabular}{ |c|c|c|c|c|c| }
 \hline \centering ID & Time & A & B & C & D \\
 \hline \centering 1 & 18:00 & ON & ON & OFF & OFF \\
 \centering 1 & 18:15 & ON & ON & OFF & OFF \\
 \centering 1 & 18:30 & ON & OFF & OFF & OFF \\
 \centering 1 & 18:45 & ON & OFF & OFF & OFF \\
 \centering 1 & 19:00 & ON & OFF & OFF & OFF \\
 \centering 1 & 19:15 & OFF & OFF & ON & OFF \\
 \centering 1 & 19:30 & OFF & OFF & ON & OFF \\
 \centering 1 & 19:45 & ON & OFF & ON & OFF \\
 \centering 1 & 20:00 & ON & OFF & ON & OFF \\
 \hline
 \centering 2 & 18:00 & ON & OFF & OFF & OFF \\
  \centering 2 & 18:15 & ON & OFF & OFF & OFF \\
 \centering 2 & 18:30 & ON & OFF & OFF & OFF \\
 \centering 2 & 18:45 & OFF & OFF & OFF & OFF \\
 \centering 2 & 19:00 & OFF & OFF & OFF & OFF \\
 \centering 2 & 19:15 & OFF & OFF & OFF & OFF \\
 \centering 2 & 19:30 & OFF & OFF & OFF & OFF \\
 \centering 2 & 19:45 & OFF & OFF & OFF & OFF \\
 \centering 2 & 20:00 & OFF  & OFF & OFF &  OFF\\
 \hline
 \centering 3 & 18:00 & ON & ON & OFF & OFF \\
 \centering 3 & 18:15 & ON & ON & OFF & OFF \\
 \centering 3 & 18:30 & ON & OFF & OFF & ON \\
 \centering 3 & 18:45 & ON & OFF & OFF & ON \\
 \centering 3 & 19:00 & ON & OFF & ON & ON \\
 \centering 3 & 19:15 & OFF & OFF & ON & ON \\
 \centering 3 & 19:30 & OFF & OFF & ON & OFF \\
 \centering 3 & 19:45 & OFF & OFF & ON & OFF \\
 \centering 3 & 20:00 & OFF & OFF & ON & OFF \\
 \hline
 \centering 4 & 18:00 & ON & OFF & OFF & OFF \\
 \centering 4 & 18:15 & ON & OFF  & OFF & OFF \\
 \centering 4 & 18:30 & ON & ON & OFF & OFF \\
 \centering 4 & 18:45 & ON & ON & OFF & OFF \\
 \centering 4 & 19:00 & ON & OFF & ON & OFF \\
 \centering 4 & 19:15 & OFF & OFF & ON & OFF \\
 \centering 4 & 19:30 & OFF & OFF & ON & OFF \\
 \centering 4 & 19:45 & OFF & OFF & ON & OFF \\
 \centering 4 & 20:00 & OFF & OFF & ON & OFF \\
 \hline
\end{tabular}
\label{tbl:SymbolDatabase1}
\end{table}

==> tableTotalExtractedPatterns.tex <==
\begin{table*}[!h]
	\vspace{-0.2in}
	\caption{Summary of Extracted Patterns}
		\vspace{-0.05in}
	\centering
	\resizebox{\textwidth}{!}{
		\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
			\hline 
			\multirow{3}{*}{Support (\%)}  & \multicolumn{16}{c|}{\bfseries Confidence (\%)}
			\\  \cline{2-17}  
			& \multicolumn{4}{c|}{\bfseries NIST}  & \multicolumn{4}{c|}{\bfseries UKDALE}   & \multicolumn{4}{c|}{\bfseries DataPort} & \multicolumn{4}{c|}{\bfseries Smart City}
			\\  \cline{2-17} 
			& {\bfseries 20} & {\bfseries 40}  & {\bfseries 60}  & {\bfseries 80} & {\bfseries 20} & {\bfseries 40}  & {\bfseries 60}  & {\bfseries 80} & {\bfseries 20} & {\bfseries 40}  & {\bfseries 60}  & {\bfseries 80} & {\bfseries 20} & {\bfseries 40}  & {\bfseries 60}  & {\bfseries 80} \\
			\hline
			\centering 20  & 519,316 & 378,896 & 69,951 & 28,912 & 126,490 & 39,629 & 10,562 & 4,231 & 310,713 & 200,179 & 11,074 & 5,012 & 1,201,723 & 1,001,354 & 121,140 & 7,164   \\  \hline
			\centering 40  & 96,952 & 96,952 & 46,793 & 14,193 & 46,193 & 26,172 & 8,240 & 4,129 & 201,561 & 140,984 & 8,928 & 4,813 & 91,241 & 90,198 & 76,014 & 6,891  \\  \hline
			\centering 60  & 29,955 & 29,955 & 29,955 & 9,608 & 11,247 & 6,221 & 5,392 & 3,921 & 9,781 & 7,229 & 6,582 & 3,827 & 13,126 & 8,712 & 6,286 & 6,140  \\  \hline
			\centering 80  & 3,568 & 3,568 & 3,568 & 3,568 & 4,832 & 4,321 & 3,251 & 3,251 & 5,492 & 4,825 & 3,981 & 3,370 & 7,018 & 6,872 & 6,002 & 6,002  \\  \hline
		\end{tabular}
	}
	\label{tbl:numberextractedPatterns}
\end{table*}

%\begin{table}
%	\caption{Generated patterns of \ref{text:datasetElectricMinute}.}
%	\centering
%	\resizebox{\columnwidth}{!}{
%		\begin{tabular}{|c|c|c|c|c|}
%			\hline
%			\multicolumn{5}{|c|}{\bfseries Patterns generated for \ref{text:datasetElectricMinute}}    
%			\\  \hline
%			{}  & {\bfseries 20\% Conf.} & {\bfseries 40\% Conf.}  & {\bfseries 60\% Conf.}  & {\bfseries 80\% Conf.} \\
%			\hline
%			\centering 20\% support & 519,316 & 378,896 & 69,951 & 28,912  \\  \hline
%			\centering 40\% support & 96,952 & 96,952 & 46,793 & 14,193  \\  \hline
%			\centering 60\% support & 29,955 & 29,955 & 29,955 & 9,608  \\  \hline
%			\centering 80\% support & 3,568 & 3,568 & 3,568 & 3,568  \\  \hline
%		\end{tabular}
%	}
%	\label{tbl:numberPatternsNIST}
%\end{table}

%\begin{table}
%	\caption{Generated patterns of \ref{text:datasetUKDALE}.}
%	\centering
%	\resizebox{\columnwidth}{!}{
%		\begin{tabular}{|c|c|c|c|c|}
%			\hline
%			\multicolumn{5}{|c|}{\bfseries Patterns generated for \ref{text:datasetUKDALE}}    
%			\\  \hline
%			{}  & {\bfseries 20\% Conf.} & {\bfseries 40\% Conf.}  & {\bfseries 60\% Conf.}  & {\bfseries 80\% Conf.} \\
%			\hline
%			\centering 20\% support & 126490 & 39629 & 10562 & 4231  \\  \hline
%			\centering 40\% support & 46193 & 26172 & 8240 & 4129  \\  \hline
%			\centering 60\% support & 11247 & 6221 & 5392 & 3921  \\  \hline
%			\centering 80\% support & 4832 & 4321 & 3251 & 3251  \\  \hline
%		\end{tabular}
%	}
%	\label{tbl:numberPatternsUKDALE}
%\end{table}
%
%\begin{table}
%	\caption{Generated patterns of \ref{text:datasetDataport}.}
%	\centering
%	\resizebox{\columnwidth}{!}{
%		\begin{tabular}{|c|c|c|c|c|}
%			\hline
%			\multicolumn{5}{|c|}{\bfseries Patterns generated for \ref{text:datasetDataport}}    
%			\\  \hline
%			{}  & {\bfseries 20\% Conf.} & {\bfseries 40\% Conf.}  & {\bfseries 60\% Conf.}  & {\bfseries 80\% Conf.} \\
%			\hline
%			\centering 20\% support & 310713 & 200179 & 11074 & 5012  \\  \hline
%			\centering 40\% support & 201561 & 140984 & 8928 & 4813  \\  \hline
%			\centering 60\% support & 9781 & 7229 & 6582 & 3827  \\  \hline
%			\centering 80\% support & 5492 & 4825 & 3981 & 3370  \\  \hline
%		\end{tabular}
%	}
%	\label{tbl:numberPatternsPecanStreet}
%\end{table}

%\begin{table}
%	\caption{Generated patterns of \ref{text:datasetMotorist}.}
%	\centering
%	\resizebox{\columnwidth}{!}{
%		\begin{tabular}{|c|c|c|c|c|}
%			\hline
%			\multicolumn{5}{|c|}{\bfseries Patterns generated for \ref{text:datasetMotorist}}    
%			\\  \hline
%			{}  & {\bfseries 20\% Conf.} & {\bfseries 40\% Conf.}  & {\bfseries 60\% Conf.}  & {\bfseries 80\% Conf.} \\
%			\hline
%			\centering 20\% support & 1201723 & 1001354 & 121140 & 7164  \\  \hline
%			\centering 40\% support & 91241 & 90198 & 76014 & 6891  \\  \hline
%			\centering 60\% support & 13126 & 8712 & 6286 & 6140  \\  \hline
%			\centering 80\% support & 7018 & 6872 & 6002 & 6002  \\  \hline
%		\end{tabular}
%	}
%	\label{tbl:numberPatternsSmartCity}
%\end{table}
